Temporal Conjunctive Query Answering in the Extended DL-Lite Family

Ontology-based query answering (OBQA) augments classical query answering in databases by domain knowledge encoded in an ontology. Systems for OBQA use the ontological knowledge to infer new information that is not explicitly given in the data. Moreover, they usually employ the open-world assumption, which means that knowledge that is not stated explicitly in the data and that is not inferred is not assumed to be true or false. Classical OBQA however considers only a snapshot of the data, which means that information about the temporal evolution of the data is not used for reasoning and hence lost. We investigate temporal conjunctive queries (TCQs) that allow to access temporal data through classical ontologies. In particular, we study combined and data complexity of TCQ entailment for ontologies written in description logics from the extended DL-Lite family. Many of these logics allow for efficient reasoning in the atemporal setting and are successfully applied in practice. We show comprehensive complexity results for temporal reasoning with these logics.

==> macros.tex <==
%!TeX root=paper.tex


\newcommand{\mycolorbox}[2]{%
\begin{tikzpicture}[baseline=(O.base)]%
	\node[fill=#1,inner sep=1pt](O){#2\vphantom{$A^I_J$}};%
\end{tikzpicture}%
}


\newcommand{\ie}{i.e.,\ }
\newcommand{\eg}{e.g.,\ }
\newcommand{\wrt}{w.r.t.\ }
\newcommand{\cf}{cf.\ }


\newcommand{\TTypes}{\ensuremath{\mathbb{T}}\xspace} %\mathsf{tType}
\newcommand{\BType}{\ensuremath{\mathsf{BT}}\xspace}
\newcommand{\Type}{\ensuremath{\mathsf{T}}\xspace}
\newcommand{\atuple}{\ensuremath{\mathsf{t}}\xspace} %\mathsf{tType}
\newcommand{\TreeAlgo}{\ensuremath{\mathsf{TreeABox}}\xspace}
\newcommand{\mypar}[1]{\medskip\noindent\textbf{#1.}}
\newcommand{\funnnit}{\ensuremath{\nu}\xspace}


% \newcommand{\fiveexp}[1]{\ensuremath{{{}^5}#1}\xspace}
\newcommand{\sizeoq}{\ensuremath{\Xi}\xspace}
\newcommand{\bound}{\ensuremath{\textsc{4-exp}(\sizeoq)}\xspace}
\newcommand{\aboxtype}[1]{\ensuremath{\Amc^+_{#1}}\xspace}
\newcommand{\typeai}[2]{\ensuremath{\smash{\Tmc^{#1}_{#2}}}\xspace}
\newcommand{\ttypea}[1]{\ensuremath{\smash{\tau^\atuple_{#1}}}\xspace}
\newcommand{\tabox}[2]{\ensuremath{\Amc^{#1}_{#2}}\xspace}




\newcommand{\rews}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Ibb}{\ensuremath{\mathbb{I}}\xspace}
\newcommand{\Abb}{\ensuremath{\mathbb{A}}\xspace}
\newcommand{\Ab}{\ensuremath{\afb^{[\aint_\akb]}}\xspace}
\newcommand{\Abr}{\ensuremath{\Ab_{\mathsf{R}}}\xspace}
\newcommand{\Abf}{\ensuremath{\afb^{\mid[\aint_\akb]}}\xspace}
\newcommand{\Abrf}{\ensuremath{\Abf_{\mathsf{R}}}\xspace}

\newcommand{\asubcontext}{\mathrm{Context}}
\newcommand{\aconceptquery}{\mathrm{C}}
%example font
\newcommand{\x}[1]{\ensuremath{\mathtt{#1}}\xspace}
\newcommand{\xs}[1]{\ensuremath{\mathsf{#1}}\xspace}

\newcommand{\cfocus}{\mathrm{Focus}}
\newcommand{\editors}{editors, }
\newcommand{\pages}{pages }


\newcommand{\xsProcess}{{Process}}
\newcommand{\xsWindow}{{Window}}
\newcommand{\xsObservation}{{Observation}}
\newcommand{\xsId}{{ID}}
\newcommand{\xsType}{{TYPE}}
\newcommand{\xsStat}{{STAT}}
\newcommand{\xsTime}{{TIME}}
\newcommand{\xsProc}{{PROC}}
\newcommand{\xsUser}{{USER}}
\newcommand{\xsObj}{{ITEM}}
\newcommand{\xsSensor}{{SENSOR}}
%\newcommand{\xsEYE}{\xs{EYE}}
%\newcommand{\xsFOC}{\xs{FOC}}
%\newcommand{\xsVID}{\xs{VID}}
%\newcommand{\xsSYS}{\xs{SYS}}
\newcommand{\xsEYE}{\x{eye}}
\newcommand{\xsFOC}{\x{foc}}
\newcommand{\xsVID}{\x{vid}}
\newcommand{\xsSYS}{\x{sys}}

\newcommand{\xcComp}{\x{Component}}
\newcommand{\xcUser}{\x{User}}
\newcommand{\xcVideo}{\x{VideoPlayer}}
\newcommand{\xcApp}{\x{Application}}
\newcommand{\xcEIntensive}{\x{EnergyIntensive}}
\newcommand{\xcRunning}{\x{Running}}
\newcommand{\xcSystemcritical}{\x{SystemCritical}}
%
\newcommand{\xcDishwasher}{\x{Dishwasher}}
\newcommand{\xcSwitchedon}{\x{SwitchedOn}}
\newcommand{\xcRoom}{\x{Room}}
\newcommand{\xcLightsoff}{\x{AllLightsOff}}
\newcommand{\xcESM}{\x{EnergySaverMode}}
\newcommand{\xcFPM}{\x{FullPowerMode}}
\newcommand{\xcDefect}{\x{Defect}}
\newcommand{\xcSCDefect}{\x{CriticalDefect}}
\newcommand{\xcOutoffoc}{\x{OutOfFocus}}

\newcommand{\xcOccupant}{\x{RoomOccupant}}
\newcommand{\xcLight}{\x{Light}}
\newcommand{\xcScreen}{\x{Screen}}
\newcommand{\xcSleeping}{\x{Sleeping}}
\newcommand{\xcSwitchedoff}{\x{SwitchedOff}}

\newcommand{\xrPartof}{\x{PartOf}}
\newcommand{\xrFocuses}{\x{FocusesOn}}
\newcommand{\xrLooksat}{\x{LooksAt}}
\newcommand{\xrWLConnectedto}{\x{WirelessConnectedTo}}
\newcommand{\xrWiredTo}{\x{WiredTo}}
\newcommand{\xrIsfilled}{\x{FilledBy}}
\newcommand{\xrHasoccupant}{\x{HasOccupant}}
\newcommand{\xrHasstate}{\x{HasState}}
\newcommand{\xrHasoffstate}{\x{HasOffState}}
\newcommand{\xrHasdevice}{\x{HasDevice}}
\newcommand{\xrHaspart}{\x{HasPart}}

\newcommand{\xsrcCompone}{\x{Window}}
\newcommand{\xsrcComptwo}{\x{Application}}
\newcommand{\xsrcCompthr}{\x{VideoPlayer}}
\newcommand{\xsrcCompfou}{\x{TextEditor}}
\newcommand{\xsrcPartofone}{\x{hasComponent}}
\newcommand{\xsrcFocusesone}{\x{LooksAt}}

\newcommand{\xiProcess}{\x{process1}}
\newcommand{\xiSystem}{\x{system}}
\newcommand{\xiUser}{\x{user}}
\newcommand{\xiBob}{\x{bob}}
\newcommand{\xiVideo}{\x{window1}}
%
\newcommand{\xiBook}{\x{book5}}
\newcommand{\xiAnn}{\x{ann}}
\newcommand{\xiWindowtwo}{\x{window4}}
\newcommand{\xiProc}{\x{p02}}
\newcommand{\xiProctwo}{\x{p01}}
%\newcommand{\xfocuses}{\x{FocusesOn}}
%\newcommand{\xfocusessrcone}{\x{LooksAt}}
%\newcommand{\pfocusessrctwo}{\x{TypesIn}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\doo}{\ensuremath{\Dmc_\aont}\xspace}
\newcommand{\doq}[1]{\ensuremath{\Dmc_\aont(#1)}\xspace}

\newcommand{\rwlem}{Lemma~}%lemma in related work
\newcommand{\cond}{Condition~}
\newcommand{\rccond}{C}

\newcommand{\domfunc}{Function~}
\newcommand{\domfuncs}{Functions~}

\newcommand{\tabthm}{Th.~}
\newcommand{\tablem}{Lem.~}
\newcommand{\tabprop}{Prop.~}
\newcommand{\tabcor}{Co.~}


\newcommand{\citethm}{Thm.~}
\newcommand{\citelem}{Lem.~}
\newcommand{\citeprop}{Prop.~}
\newcommand{\citecor}{Cor.~}
\newcommand{\citech}{Ch.~}
\newcommand{\citesec}{Sec.~}
\newcommand{\citefig}{Fig.~}
\newcommand{\rwlems}{Lemmas~}

\newcommand{\arule}{\ensuremath{\sigma}\xspace}

\newcommand{\ggci}{\ensuremath{_{\mid gGCI}}\xspace}

\newcommand{\QL}{\ensuremath{\mathcal{QL}}\xspace}
\newcommand{\adl}{\ensuremath{\mathcal{DL}}\xspace}
\newcommand{\atl}{\ensuremath{\mathcal{TL}}\xspace}


\newcommand{\SQL}{\textbf{SQL}\xspace}
\newcommand{\Datalog}{\textbf{Datalog}\xspace}
\newcommand{\LTL}{\textnormal{{LTL}}\xspace}%\textbf{LTL}}\xspace}
\newcommand{\FO}{FO\xspace}
\newcommand{\FOL}{\textbf{FOL}\xspace}
\newcommand{\algofont}[1]{\texttt{#1}}

\newcommand{\algoComputeQueryEntailment}{\algofont{computeQueryEntailment}\xspace}
\newcommand{\algoUnify}{\algofont{unify}\xspace}

\newcommand{\obda}{OBDA\xspace}

\newcommand{\algoPreprocessing}{PREPROCESS}
\newcommand{\algoGuessing}{GUESSDATA}
\newcommand{\algoTesting}{RSATISFIABLE}

\newcommand{\algoELCQNEnt}{CQNOTENTAILED}
\newcommand{\algoELKBCons}{KBCONSISTENT}
\newcommand{\algoELWits}{WITNESSENUM}


\newcommand{\algoDllhhornUCQEnt}{UCQENTAILED}
\newcommand{\algoDllhhornKBCons}{KBCONSISTENT}
\newcommand{\algoDllhhornWQs}{WITNESSQENUM}
\newcommand{\algoDllhhornTreeShaped}{TREEWITNESSENUM}
\newcommand{\algoCQConseqs}{CQCONSEQUENCES}

\newcommand{\algoBoolCons}{CONSISTENT}%\xspace}
\newcommand{\algoTCons}{TCOMPATIBLE}
\newcommand{\algoInitial}{INITIAL}

\newcommand{\fnow}{{pres}}
\newcommand{\fnext}{{next}}
\newcommand{\fs}{s}

\newcommand{\algoDllhhornCons}{\textsf{Consistent}\xspace}
%\newcommand{\algoDllhhornRew}{\textsf{PerfectRef}\xspace}
\newcommand{\dbint}{\dboa}%DB\xspace

%\newcommand{\dllhhornQUnsat}[1]{\ensuremath{\mathsf{Consistent}(#1)}\xspace}
\newcommand{\dllhhornQUnsat}[1]{\ensuremath{q_{unsat(#1)}}\xspace}%\ensuremath{\mathsf{Consistent}(#1)}\xspace}
\newcommand{\dllhhornPerfRef}[2]{\ensuremath{q_{ref(#1,#2)}\xspace}}
%{\ensuremath{\mathsf{PerfectRef}(#1,#2)}\xspace}%Q, ont

\newcommand{\adatalogprog}{\ensuremath{P}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%basic syntax LOGIC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\asymbol}{\ensuremath{X}\xspace}
\newcommand{\vtwo}{\ensuremath{y}\xspace}
\newcommand{\vthr}{\ensuremath{z}\xspace}
\newcommand{\aplform}{\ensuremath{\varphi}\xspace}%propositional logic
\newcommand{\afoform}{\ensuremath{\varphi}\xspace}%propositional logic

%\newcommand{\aterm}{\ensuremath{t}\xspace}
\newcommand{\tone}{\ensuremath{s}\xspace}
\newcommand{\ttwo}{\ensuremath{t}\xspace}
\newcommand{\tthr}{\ensuremath{u}\xspace}

\newcommand{\amonoid}{\ensuremath{M}\xspace}%\mathfrac{M}}\xspace}%\mathsf{Sub}}\xspace}

% \newcommand{\formsub}[1]{\ensuremath{\mathbb{F}(#1)}\xspace}%\mathsf{Sub}}
% \newcommand{\Subform}{\ensuremath{\mathbb{S}}\xspace}%\mathsf{Sub}}\xspace}

\newcommand{\domain}{\ensuremath{\mathsf{domain}}\xspace}
\newcommand{\range}{\ensuremath{\mathsf{range}}\xspace}

\newcommand{\pa}[1]{\ensuremath{#1^{\smash{\mathrm{pa}}}}\xspace}
\newcommand{\pba}[1]{\ensuremath{#1^{\smash{\mathrm{ba}}}}\xspace}%\ensuremath{#1^\mathsf{ba}}\xspace}

\newcommand{\val}{\ensuremath{v}\xspace} % a valuation
\newcommand{\ahom}{\ensuremath{\pi}\xspace}
\newcommand{\ahomtwo}{\ensuremath{\pi'}\xspace}
\newcommand{\ahomthr}{\ensuremath{\tau}\xspace}

%\newcommand{\proofcase}[1]{#1.\  }
%\newcommand{\proofcase}[1]{\textbf{Case #1:}  }





\newcommand{\eps}{\epsilon}
\newcommand{\true}{\ensuremath{\mathit{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathit{false}}\xspace}


\newcommand{\atopform}{\ensuremath{f}\xspace}
\newcommand{\atopfone}{\ensuremath{f}\xspace}
\newcommand{\atopftwo}{\ensuremath{g}\xspace}
\newcommand{\atype}{\ensuremath{T}\xspace}
\newcommand{\atypeset}[1][\Pmc]{\ensuremath{\mathsf{Typ}(#1)}\xspace}
\newcommand{\Clo}{\ensuremath{\mathsf{Clo}}\xspace}
\newcommand{\atmfut}[2]{\ensuremath{\mathrm{Fut}_{(#1,#2)}}\xspace}
%\newcommand{\atmpast}[2]{\ensuremath{\mathrm{Past}_{(#1,#2)}}\xspace}


\newcommand{\afformset}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\apformset}{\ensuremath{\mathcal{P}}\xspace}




\newcommand{\asignature}{\ensuremath{\Sigma}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%basic syntax DL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\term}{\NT}%\mathsf{term}}\xspace}


\newcommand{\adlsignature}{\ensuremath{\Sigma}\xspace}
\newcommand{\aname}{\ensuremath{X}\xspace}
\newcommand{\acone}[1][]{\ensuremath{C^{\smash{#1}}}\xspace}
\newcommand{\actwo}[1][]{\ensuremath{D^{\smash{#1}}}\xspace}%TODO replace by CD
\newcommand{\rone}{\ensuremath{R_1}\xspace}
\newcommand{\rtwo}{\ensuremath{R_2}\xspace}%TODO replace by RS
\newcommand{\indone}{\ensuremath{a}\xspace}
\newcommand{\indtwo}{\ensuremath{b}\xspace}%{\tiny'}}\xspace}
%TODO replace by ab
\newcommand{\el}{\ensuremath{e}\xspace}
\newcommand{\eladd}{\ensuremath{d}\xspace}
\newcommand{\elone}{\ensuremath{d}\xspace}
\newcommand{\eltwo}{\ensuremath{e}\xspace}%e{\tiny'}
\newcommand{\abcset}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\aaxiom}{\ensuremath{\alpha}\xspace}
\newcommand{\aelaxiom}{\aaxiom}
\newcommand{\aont}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\atheory}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\afb}{\ensuremath{\mathcal{A}}\xspace}

\newcommand{\akb}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\aint}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\fin}{\ensuremath{^{\smash f}}\xspace}
\newcommand{\adom}[1][]{\ensuremath{\Delta^{{#1}}}\xspace}
\newcommand{\Ans}{\ensuremath{\mathsf{Ans}}\xspace}
\newcommand{\Cert}{\ensuremath{\mathsf{Cert}}\xspace}

\newcommand{\un}{\ensuremath{\mathsf{u}}\xspace}
\newcommand{\apath}{\ensuremath{\varrho}\xspace}
\newcommand{\apathtwo}{\ensuremath{\sigma}\xspace}

\newcommand{\BC}{\ensuremath{\mathbb{B}}\xspace}%\mathsf{BC}}\xspace}
% \newcommand{\BCn}{\ensuremath{\mathbb{C}}\xspace}%\BC^\lnot}\xspace}
\newcommand{\ontsub}[1][\aont]{\ensuremath{\mathbb{S}(\aont)}\xspace}%\mathrm{Sub}_{#1}}\xspace}
% \newcommand{\Sub}{\ensuremath{\mathbb{S}}\xspace}%\mathsf{SC}}\xspace}
\newcommand{\AS}{\ensuremath{\mathbb{A}}\xspace}

%\newcommand{\Subq}{\ensuremath{\mathbb{S}}\xspace}%\mathsf{SC}}\xspace}
\newcommand{\qsub}{\ensuremath{\mathbb{S}}\xspace}%\mathsf{SC}}\xspace}
\newcommand{\Flat}{\ensuremath{\BC(\aont)}\xspace}
%	\ensuremath{\mathbb{F}(\aont)}\xspace}%\mathsf{SC}}\xspace}
\newcommand{\FlatR}{\BCr}
%	\ensuremath{\mathbb{F}_\mathsf{R}}\xspace}%\mathsf{SC}}\xspace}


\newcommand{\DB}{\ensuremath{\mathsf{DB}}\xspace}
\newcommand{\TDB}{\ensuremath{\mathsf{TDB}}\xspace}

\newcommand{\io}{\ensuremath{\aint_\akb}\xspace}
\newcommand{\iof}{\ensuremath{\aint_\akb^{\smash f}}\xspace}
\newcommand{\ior}{\smash{\ensuremath{\aint'_\akb}}\xspace}
\newcommand{\iorit}[1]{\smash{\ensuremath{\aint'_{\akb,#1}}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%basic syntax LTL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\apropset}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\altlsignature}{\apropset}%{\ensuremath{\Sigma}\xspace}
\newcommand{\altlform}{\ensuremath{\varphi}\xspace}
\newcommand{\altlformtwo}{\ensuremath{\psi}\xspace}
\newcommand{\altlint}{\ensuremath{\Wmf}\xspace}

\newcommand{\alllits}[1]{\ensuremath{\mathrm{Lit}_#1}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%basic syntax QA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\aquery}{\ensuremath{\varphi}\xspace}
\newcommand{\aquerytwo}{\ensuremath{\psi}\xspace}%rho
\newcommand{\aq}{\aquery}
\newcommand{\acq}{\aquery}
\newcommand{\acqtwo}{\aquerytwo}
\newcommand{\acqthr}{\ensuremath{\sigma}\xspace}
\newcommand{\aatom}{\ensuremath{\aaxiom}\xspace}
\newcommand{\aans}{\ensuremath{\mathfrak{a}}\xspace}

\newcommand{\Q}{\ensuremath{Q}\xspace}% a set of CQs

\newcommand{\cqinst}[1]{\ensuremath{\afb_{#1}}\xspace} 
\newcommand{\cqgraph}[1]{\ensuremath{\mathrm{G}_{#1}}\xspace}%\mathcal{G}_{#1}}\xspace}

\newcommand{\cqcon}[1]{\ensuremath{\mathrm{Con}(#1)}\xspace} %EL
\newcommand{\cqconr}[2]{\ensuremath{\mathrm{Con'}(#1,#2)}\xspace} %EL  +root var
\newcommand{\cqcontw}[3]{\ensuremath{\mathrm{Con}_{#1}(#2,#3)}\xspace} %DLL

%TODO remove because often use directly anyway
\newcommand{\FVar}{ \NFV}%\ensuremath{\mathsf{FVar}}\xspace}
\newcommand{\Var}{ \NV}%\ensuremath{\mathsf{Var}}\xspace}
\newcommand{\Ind}{\NI}
\newcommand{\At}{\ensuremath{\mathsf{At}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%syntax TQA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\afbs}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\atkb}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\atcq}{\ensuremath{\Phi}\xspace}
\newcommand{\atcqtwo}{\ensuremath{\Psi}\xspace}
\newcommand{\aelltlform}{\atcq}
\newcommand{\aelltlformtwo}{\atcqtwo}
\newcommand{\atq}{\ensuremath{\atcq}\xspace}
\newcommand{\atqtwo}{\ensuremath{\atcqtwo}\xspace}
\newcommand{\atint}{\ensuremath{\mathfrak{I}}\xspace}


\newcommand{\as}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\ax}{\ensuremath{W}\xspace}%\ensuremath{\omega}\xspace}%\ensuremath{\mathcal{W}}}

\newcommand{\pv}{{\ensuremath{\{p_1,\dots,p_m\}}}\xspace}

\newcommand{\acqalpha}{\ensuremath{\acq}\xspace}%a specific cq
\newcommand{\acqalphatwo}{\ensuremath{\acq'}\xspace}%a specific cq
\newcommand{\aalpha}{\acqalpha}%{\ensuremath{\alpha}\xspace}%in elltl

\newcommand{\tcqcqs}[1]{\ensuremath{\mathcal{Q}_{#1}}\xspace} %\mathrm{CQ}(#1)}\xspace}%

\newcommand{\BR}{\ensuremath{\Bmc|_\mathsf{R}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%syntax R-COMPLETE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tw}[1][]{\ensuremath{\mathrm{f}_{#1}}\xspace}
\newcommand{\atwrset}{\ensuremath{\ensuremath{\mathcal{R}}}\xspace}%dll tree witness 

% \newcommand{\acwit}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\awit}{\ensuremath{\mathcal{B}_\mathsf{R}}\xspace} %= a cq wit
\newcommand{\wits}[2]{\ensuremath{\mathcal{W}_{#1}(#2)}\xspace}

\newcommand{\cqcons}{\ensuremath{\Cmc_\Omc}\xspace} %TODO make func

\newcommand{\BCr}{\ensuremath{\BC_\mathsf{R}}\xspace}
\newcommand{\BCf}{\ensuremath{\BC_\mathsf{F}}\xspace}
% \newcommand{\BCrn}{\ensuremath{\BCn_\mathsf{R}}\xspace}
%\newcommand{\BCrn}{\ensuremath{\BCr^\lnot}\xspace}
\newcommand{\ASr}{\ensuremath{\AS_\mathsf{R}}\xspace}
\newcommand{\ASf}{\ensuremath{\AS_\mathsf{F}}\xspace}

\newcommand{\NIA}{\ensuremath{\mathsf{N}^{\mathsf{aux}}_{\mathsf{I}}}\xspace}
\newcommand{\NIT}{\ensuremath{\mathsf{N}^{\mathsf{tree}}_{\mathsf{I}}}\xspace}
\newcommand{\NITm}{\ensuremath{\mathsf{N}^{\mathsf{tree}-}_{\mathsf{I}}}\xspace}

\newcommand{\AR}{\ensuremath{\Amc_{\mathsf{R}}}\xspace}
\newcommand{\ARex}{\ensuremath{\Amc_{\smash{\mathsf{R}}}^{\tiny\exists}}\xspace}
\newcommand{\QR}{\ensuremath{Q_\mathsf{R}}\xspace} %
\newcommand{\QRn}{\ensuremath{Q^{\smash\neg}_{\smash{\mathsf{R}}}}\xspace} %
\newcommand{\RF}[1][]{\ensuremath{\Rmc_{\mathsf{F}#1}}\xspace}%{\ensuremath{R_\mathsf{F}}\xspace}
\newcommand{\KR}[1][]{\ensuremath{\akb_{\mathsf{rc}}^{#1}}\xspace}

\newcommand{\chiR}{\ensuremath{\chi_\mathsf{R}}\xspace} 
\newcommand{\chij}{\ensuremath{\chi_\mathsf{q(j)}}\xspace} 


%\newcommand{\adomp}[2][]{\ensuremath{\adom[#1]_{\smash{#2}}}\xspace}% a dom part


\newcommand{\adomp}[2][]{\ensuremath{\adom[#1]_{\smash{#2}}}\xspace}% a dom part
\newcommand{\unR}{\ensuremath{\mathsf{u_R}}\xspace}
\newcommand{\aux}{\ensuremath{\mathsf{a}}\xspace}
\newcommand{\tree}{\ensuremath{\mathsf{t}}\xspace}
\newcommand{\nam}{\ensuremath{\mathsf{n}}\xspace}

%
\newcommand{\ael}[2][]{\ensuremath{a_{\smash{#2}}^{\smash{#1}}}\xspace}
\newcommand{\aiel}[1]{\ensuremath{a^{\smash i}_{\smash{#1}}}\xspace}
\newcommand{\ajel}[1]{\ensuremath{a^{\smash j}_{\smash{#1}}}\xspace}
%
\newcommand{\uel}[2][]{\ensuremath{u_{\smash{#2}}^{\smash{#1}}}\xspace}
\newcommand{\uiel}[1]{\ensuremath{u^{\smash i}_{\smash{#1}}}\xspace}
\newcommand{\ujel}[1]{\ensuremath{u^{\smash j}_{\smash{#1}}}\xspace}
\newcommand{\upel}[1]{\ensuremath{u'_{\smash{#1}}}\xspace}%uprime el


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%proof DOMINO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ds}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dsD}{\ensuremath{T}\xspace}
\newcommand{\dsH}{\ensuremath{H}\xspace}
\newcommand{\dsV}{\ensuremath{V}\xspace}
\newcommand{\dsI}{\ensuremath{I}\xspace}
\newcommand{\dsd}{\ensuremath{t}\xspace}

\newcommand{\dsh}{\ensuremath{^{\smash h}}\xspace}
\newcommand{\dsv}{\ensuremath{^{\smash v}}\xspace}
\newcommand{\dsL}{\ensuremath{L_{\smash t}}\xspace}
\newcommand{\dsG}{\ensuremath{G_{\smash t}}\xspace}
\newcommand{\dsGo}{\ensuremath{G}\xspace}
\newcommand{\dsGh}{\ensuremath{G_{\smash t}\dsh}\xspace}
\newcommand{\dsGv}{\ensuremath{G_{\smash t}\dsv}\xspace}

\newcommand{\hor}{\ensuremath{^{\smash h}}\xspace}
\newcommand{\ver}{\ensuremath{^{\smash v}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%proof AUTOMATA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\aautom}[1][]{\ensuremath{\mathfrak{M}_{#1}}\xspace}
\newcommand{\atm}[1][]{\ensuremath{\mathfrak{M}_{#1}}\xspace}%[\aont,\atcq]
\newcommand{\tm}[1]{\ensuremath{\mathfrak{M}_{#1}}\xspace}%[\aont,\atcq]


\newcommand{\automQ}{\ensuremath{Q}\xspace}
\newcommand{\automA}{\ensuremath{\Sigma}\xspace}
\newcommand{\automT}{\ensuremath{\Delta}\xspace}
\newcommand{\automqs}{\ensuremath{q_0}\xspace}
\newcommand{\automF}{\ensuremath{F}\xspace}



%TODO WHATs THAT? - check if still needed and replace by better names
\newcommand{\An}{\ensuremath{A^\mathsf{n}}\xspace}


\newcommand{\rigctypes}{\ensuremath{\Tmc}\xspace}
\newcommand{\rigctype}{\ensuremath{T}\xspace}


\newcommand{\Con}[1][]{\ensuremath{\mathsf{con}_{#1}}\xspace}
\newcommand{\ConR}{\ensuremath{\mathsf{Con^R}}\xspace}

\newcommand{\rsimple}{r-simple\xspace}


\newcommand{\ind}{\ensuremath{\mathsf{|n}}\xspace}

\newcommand{\Lit}{\ensuremath{\mathsf{Lit}}\xspace}
\newcommand{\wit}{\ensuremath{\mathsf{wit}}\xspace}

\newcommand{\Ochi}{\ensuremath{\Omc_\chi}\xspace}
\newcommand{\nc}[1]{\ensuremath{nc(#1)}\xspace}
\newcommand{\pr}[2]{\ensuremath{#1^{#2}}\xspace}
\newcommand{\tpr}[2]{\ensuremath{#1^{#2}}\xspace}

%\let\oldDelta\Delta
%\renewcommand{\Delta}{\mathrm{\oldDelta}}

\newcommand{\Cl}{\ensuremath{\mathsf{Cl}}\xspace}


\newcommand{\CAT}{\ensuremath{\mathsf{CAt}}\xspace}
\newcommand{\RAT}{\ensuremath{\mathsf{RAt}}\xspace}
\newcommand{\SC}{\ensuremath{\mathsf{SC}}\xspace}
\newcommand{\SCN}{\ensuremath{\mathsf{SC}_\neg}\xspace}
\newcommand{\TR}[1][]{\ensuremath{\Tmc_\mathsf{R}^{#1}}\xspace}
\newcommand{\SubR}{\ensuremath{\mathsf{Sub_R}}\xspace}
\newcommand{\ty}{\ensuremath{\mathbb{t}}\xspace}
\newcommand{\tyR}{\ensuremath{\mathsf{t}_\mathsf{R}}\xspace}



% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% REWRITING
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\newcommand{\tpparam}{\ensuremath{i}\xspace}%MUST REFER TO I somehow
\newcommand{\tdboa}{\TDB\xspace}
\newcommand{\tdbfbs}{\tdb{\afbs}}
\newcommand{\tdb}[1]{\ensuremath{\TDB(#1)}\xspace}%\ensuremath{TDB(#1)}\xspace}
\newcommand{\dboa}{{\DB}\xspace}
\newcommand{\db}[1]{\ensuremath{\DB(#1)}\xspace}%
\newcommand{\A}{\ensuremath{\mathsf{A}}\xspace}
\newcommand{\B}{\ensuremath{\mathsf{B}}\xspace}
\newcommand{\R}{\ensuremath{\mathsf{R}}\xspace}
\newcommand{\Adb}{\ensuremath{\mathsf{A^\dboa}}\xspace}
\newcommand{\Bdb}{\ensuremath{\mathsf{B^\dboa}}\xspace}
\newcommand{\Rdb}{\ensuremath{\mathsf{R^\dboa}}\xspace}

\newcommand{\KRis}[1][]{\ensuremath{\Kmc_{\mathsf{rc}\SRdep}^{i}}\xspace}%\smash{\mathsf{R}\SRdep}
\newcommand{\AKRis}{\ensuremath{{\Amc^i_{\mathsf{rc}\SXRdep}}}\xspace}%_{{\Kmc_{\mathsf{R}}^{i}\SRdep}}}\xspace}%\smash
% \newcommand{\AKRisp}{\ensuremath{{\Amc^{i\mid\prot}_{\mathsf{rc}\SXRdep}}}\xspace}%_{{\Kmc_{\m

\newcommand{\Sdep}{\ensuremath{[\as]}\xspace} %
\newcommand{\SRdep}{\ensuremath{[\as,\Bphi]}\xspace} 
\newcommand{\SXRdep}{\ensuremath{[\as,\ax,\Bphi]}\xspace} 
\newcommand{\Rdep}{\ensuremath{[\Bphi]}\xspace} 

% \newcommand{\Brphi}{\ensuremath{\Bmc_{\atcq\mathsf{\mid R}}}\xspace}
\newcommand{\Bphi}{\ensuremath{\Bmc_\atcq}\xspace}
% \newcommand{\Bro}{\ensuremath{\Bmc_\mathsf{o\mid R}}\xspace}
% \newcommand{\Bo}{\ensuremath{\Bmc_\mathsf{o}}\xspace}

\newcommand{\QRs}{\ensuremath{Q_{\mathsf{R}\Sdep}}\xspace} %
\newcommand{\QRsn}{\ensuremath{Q^\neg_{\smash{\mathsf{R}\Sdep}}}\xspace} %
\newcommand{\ARs}{\ensuremath{\Amc_{\mathsf{R}\smash{\SRdep}}}\xspace}
\newcommand{\RFs}{\ensuremath{\RF[\SRdep]}\xspace}
\newcommand{\RFaux}{\ensuremath{\RF[\mid\auxp\Sdep]}\xspace}
\newcommand{\RFpro}{\ensuremath{\RF[\mid\pro]}\xspace}
\newcommand{\RFphi}{\ensuremath{\RF[\mid\atcq\Rdep]}\xspace}
\newcommand{\RFother}{\ensuremath{\RF[\mid\mathsf{o}]}\xspace}

\newcommand{\treep}{\ensuremath{\mathsf{tree}}\xspace}
\newcommand{\auxp}{\ensuremath{\mathsf{aux}}\xspace}
\newcommand{\pro}{\ensuremath{\mathsf{pro}}\xspace}

\newcommand{\prot}{\wp}%pro transl


%TODO acq should maybe be acqalpha
\newcommand{\pref}{\ensuremath{\mathsf{PR}}\xspace}
\newcommand{\prefo}[1][\acq]{\ensuremath{\pref^{#1,\Omc}}\xspace}
% \newcommand{\preft}[2][\acq]{\ensuremath{\pref^{#1,\Omc}_{\Bro^{#2}}}\xspace}
\newcommand{\prefth}[2][\acq]{\ensuremath{\pref^{#1,\Omc}_{\ARs^{#2}}}\xspace}

\newcommand{\NIP}{\ensuremath{\mathsf{N}^{\mathsf{pro}}_{\mathsf{I}}}\xspace}
\newcommand{\NITK}{\ensuremath{\mathsf{N}^{\mathsf{tree}}_{\mathsf{I}}}\xspace}


\newcommand{\rewQUnsat}[1][i]{\ensuremath{q^{unsat(\aont)}_{ \as,\ax,\Bphi}(#1)}\xspace}
\newcommand{\rewPRef}[2][i]{\ensuremath{\pref^{#2,\aont}_{\as,\ax,\Bphi}(#1)}\xspace}%Q, 

\newcommand{\filter}{\ensuremath{\mathsf{filter}}\xspace}

% \newcommand{\rep}[2][i]{\ensuremath{\mathsf{rep}^{#2}_{\as,\ax,\Bphi}(#1)}\xspace}
% \newcommand{\repone}[2][i]{\ensuremath{\mathsf{rep}^{#2,1}_{\as,\ax,\Bphi}(#1)}\xspace}
% \newcommand{\reptwo}[2][i]{\ensuremath{\mathsf{rep}^{#2,2}_{\as,\ax,\Bphi}(#1)}\xspace}
% \newcommand{\repthree}[2][i]{\ensuremath{\mathsf{rep}^{#2,3}_{\as,\ax,\Bphi}(#1)}\xspace}
\newcommand{\repo}[1]{\ensuremath{\lfloor #1\rfloor}\xspace}
\newcommand{\rep}[2][i]{\ensuremath{\repo{#2}(#1)}\xspace}
\newcommand{\repone}[2][i]{\ensuremath{\repo{#2}^1(#1)}\xspace}
\newcommand{\reptwo}[2][i]{\ensuremath{\repo{#2}^2(#1)}\xspace}
\newcommand{\repthree}[2][i]{\ensuremath{\repo{#2}^3(#1)}\xspace}
\newcommand{\rept}[3][i]{\ensuremath{\repo{#2}_{\Bro^{#3}}(#1)}\xspace}
\newcommand{\repth}[2][i]{\ensuremath{\repo{#2}_{\ARs}(#1)}\xspace}

\newcommand{\rsat}[1][\ax]{\ensuremath{\mathsf{rSat}_{\as,#1,\Bphi}}\xspace}
%\newcommand{\cons}{\ensuremath{f_{\text{(\rccond1)}}}\xspace}
%\newcommand{\answit}{\ensuremath{f_{\text{(\rccond5)}}}\xspace}
%\newcommand{\ansx}{\ensuremath{f_{\text{(\rccond2)}}}\xspace}
\newcommand{\cons}{\ensuremath{f_{\text{\rccond1}}}\xspace}
\newcommand{\answit}{\ensuremath{f_{\text{\rccond5}}}\xspace}
\newcommand{\ansx}{\ensuremath{f_{\text{\rccond2}}}\xspace}

\newcommand{\ground}{\ensuremath{\gamma}\xspace}




% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% LETTERS
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

%cal letters
\newcommand{\Amc}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Bmc}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\Cmc}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Dmc}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Emc}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\Fmc}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Gmc}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\Hmc}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\Imc}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Jmc}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\Kmc}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\Lmc}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Mmc}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Nmc}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\Omc}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\Pmc}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Qmc}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\Rmc}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Smc}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\Tmc}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Umc}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Vmc}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\Wmc}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\Xmc}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Ymc}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Zmc}{\ensuremath{\mathcal{Z}}\xspace}



%frak letters
\newcommand{\amf}{\ensuremath{\mathfrak{a}}\xspace}
\newcommand{\bmf}{\ensuremath{\mathfrak{b}}\xspace}
\newcommand{\cmf}{\ensuremath{\mathfrak{c}}\xspace}
\newcommand{\emf}{\ensuremath{\mathfrak{e}}\xspace}
\newcommand{\fmf}{\ensuremath{\mathfrak{f}}\xspace}
\newcommand{\vmf}{\ensuremath{\mathfrak{v}}\xspace}

\newcommand{\Amf}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\Cmf}{\ensuremath{\mathfrak{C}}\xspace}
\newcommand{\Fmf}{\ensuremath{\mathfrak{F}}\xspace}
\newcommand{\Imf}{\ensuremath{\mathfrak{I}}\xspace}
\newcommand{\Jmf}{\ensuremath{\mathfrak{J}}\xspace}
\newcommand{\Mmf}{\ensuremath{\mathfrak{M}}\xspace}
\newcommand{\Rmf}{\ensuremath{\mathfrak{R}}\xspace}
\newcommand{\Smf}{\ensuremath{\mathfrak{S}}\xspace}
\newcommand{\Tmf}{\ensuremath{\mathfrak{T}}\xspace}
\newcommand{\Wmf}{\ensuremath{\mathfrak{W}}\xspace}

%bb letters
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Qbb}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Xbb}{\ensuremath{\mathbb{X}}\xspace}

%bf letters
\newcommand{\cbf}{\ensuremath{\mathbf{c}}\xspace}
\newcommand{\dbf}{\ensuremath{\mathbf{d}}\xspace}
\newcommand{\fbf}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\tbf}{\ensuremath{\mathbf{t}}\xspace}
\newcommand{\Qbf}{\ensuremath{\mathbf{Q}}\xspace}
%\newcommand{\vbf}{\ensuremath{\mathbf{v}}\xspace}

%sfletters
\newcommand{\Asf}{\ensuremath{\mathsf{A}}\xspace}
\newcommand{\Nsf}{\ensuremath{\mathsf{N}}\xspace}


%DLs
\newcommand{\TDLLite}{\ensuremath{T_{\mathcal{US}}\DLLite_{bool}}\xspace}
\newcommand{\QTLO}{\ensuremath{\mathcal{QTL}^1}\xspace}
\newcommand{\PTL}{\ensuremath{\mathcal{PTL}}\xspace}
\newcommand{\DL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\EL}{\ensuremath{\mathcal{E\!L}}\xspace}
%\newcommand{\ELbot}{\ensuremath{\mathcal{EL}_\bot}\xspace}
%\newcommand{\ELObot}{\ensuremath{\mathcal{ELO}_\bot}\xspace}
%\newcommand{\ELp}{\ensuremath{\mathcal{EL}^{+}}\xspace}
%\newcommand{\ELpp}{\ensuremath{\mathcal{EL}^{++}}\xspace}
\newcommand{\ALC}{\ensuremath{\mathcal{ALC}}\xspace}
\newcommand{\ALCH}{\ensuremath{\mathcal{ALCH}}\xspace}
\newcommand{\ALCcap}{\ensuremath{\mathcal{ALC}^\cap}\xspace}
\newcommand{\SHQ}{\ensuremath{\mathcal{SHQ}}\xspace}
\newcommand{\SHOQ}{\ensuremath{\mathcal{SHOQ}}\xspace}
\newcommand{\SHIQ}{\ensuremath{\mathcal{SHIQ}}\xspace}
\newcommand{\SROIQ}{\ensuremath{\mathcal{SROIQ}}\xspace}
%\newcommand{\SHOIQ}{\ensuremath{\mathcal{SHOIQ}}\xspace}
\newcommand{\DLLite}{\textit{DL-Lite}\xspace}
\newcommand{\DLLiteh}{\ensuremath{\textit{DL-Lite}^{\mathcal{H}}}\xspace}
\newcommand{\DLLiter}{\ensuremath{\textit{DL-Lite}_{\mathcal{R}}}\xspace}
\newcommand{\DLLitehcore}{\ensuremath{\textit{DL-Lite}^\Hmc_{\textit{core}}}\xspace}
\newcommand{\DLLitecore}{\ensuremath{\textit{DL-Lite}_{\textit{core}}}\xspace}
\newcommand{\DLLitebool}{\ensuremath{\textit{DL-Lite}_{\textit{bool}}}\xspace}
\newcommand{\DLLitehbool}{\ensuremath{\textit{DL-Lite}^\Hmc_{\textit{bool}}}\xspace}
\newcommand{\DLLitehkrom}{\ensuremath{\textit{DL-Lite}^\Hmc_{\textit{krom}}}\xspace}
\newcommand{\DLLitekrom}{\ensuremath{\textit{DL-Lite}_{\textit{krom}}}\xspace}
\newcommand{\DLLitehhorn}{\ensuremath{\textit{DL-Lite}^\Hmc_{\textit{horn}}}\xspace}
\newcommand{\DLLitehorn}{\ensuremath{\textit{DL-Lite}_{\textit{horn}}}\xspace}


% complexities
\newcommand{\ExpTime}{\ensuremath{\textsc{ExpTime}}\xspace}
\newcommand{\NExpTime}{\ensuremath{\textsc{NExpTime}}\xspace}
\newcommand{\TwoExpTime}{\ensuremath{\textsc{2-ExpTime}}\xspace}
\newcommand{\NP}{\ensuremath{\textsc{NP}}\xspace}
\newcommand{\coNP}{\ensuremath{\textsc{co-NP}}\xspace}
\newcommand{\coNExpTime}{\ensuremath{\textsc{co-NExpTime}}\xspace}
\newcommand{\PTime}{\ensuremath{\textsc{P}}\xspace}
\newcommand{\PSpace}{\ensuremath{\textsc{PSpace}}\xspace}
\newcommand{\NPSpace}{\ensuremath{\textsc{NPSpace}}\xspace}
\newcommand{\ExpSpace}{\ensuremath{\textsc{ExpSpace}}\xspace}
\newcommand{\TwoExpSpace}{\ensuremath{\textsc{2-ExpSpace}}\xspace}
\newcommand{\ACi}[1][i]{\ensuremath{\textsc{AC}^{#1}}\xspace}
\newcommand{\NCi}[1][i]{\ensuremath{\textsc{NC}^{#1}}\xspace}
\newcommand{\ACzero}{\ensuremath{\textsc{AC}^0}\xspace}
\newcommand{\ACone}{\ensuremath{\textsc{AC}^1}\xspace}
\newcommand{\NCone}{\ensuremath{\textsc{NC}^1}\xspace}
\newcommand{\NLogSpace}{\ensuremath{\textsc{NLogSpace}}\xspace}
\newcommand{\LogSpace}{\ensuremath{\textsc{LogSpace}}\xspace}
\newcommand{\ALogTime}{\ensuremath{\textsc{ALogTime}}\xspace}
\newcommand{\DLogTime}{\ensuremath{\textsc{LogTime}}\xspace}
\newcommand{\LogTime}{\ensuremath{\textsc{LogTime}}\xspace}
\newcommand{\NLogTime}{\ensuremath{\textsc{NLogTime}}\xspace}
\newcommand{\PiTwoP}{\ensuremath{\Pi^\text{\upshape{P}}_2}\xspace}

% maths


% temporal operators
\newcommand{\Nextstar}{\ensuremath{\ocircle_*}\xspace}
\newcommand{\Next}{\ensuremath{\ocircle_F}\xspace}
\newcommand{\WNext}{\raisebox{-.4ex}{\scalebox{1.7}{\ensuremath{\bullet}}\ensuremath{_F}}
\xspace }
%\newcommand{\sWNext}{\raisebox{-.4ex}{\scalebox{1.35}{\ensuremath{\bullet}}}
%\xspace }
\newcommand{\Previous}{\ensuremath{\ocircle_P}\xspace}%\Next^-}\xspace}
\newcommand{\WPrevious}{\raisebox{-.4ex}{\scalebox{1.7}{\ensuremath{\bullet}}\ensuremath{_P}}
	\xspace }
%\newcommand{\sWPrevious}{\ensuremath{\sWNext^-}\xspace}
% \newcommand{\Since}{\ensuremath{\mathsf{S}}\xspace}
\DeclareMathOperator*{\Since}{\mathcal{S}}
% \newcommand{\sSince}{\ensuremath{\mathsf{S}^<}\xspace}
\DeclareMathOperator*{\sSince}{\mathcal{S}^<}
% \newcommand{\Until}{\ensuremath{\mathsf{U}}\xspace}
\DeclareMathOperator*{\Until}{\mathcal{U}}%\mathsf{U}} %\mathsf{U}}
% \newcommand{\sUntil}{\ensuremath{\mathsf{U}^<}\xspace}
\DeclareMathOperator*{\sUntil}{\mathcal{U}^<}
\newcommand{\Diamondf}{\ensuremath{\Diamond_F}\xspace}
\newcommand{\Boxf}{\ensuremath{\Box_F}\xspace}
\newcommand{\Diamondm}{\ensuremath{\Diamond_P}\xspace}
\newcommand{\Boxm}{\ensuremath{\Box_P}\xspace}
\newcommand{\first}{\ensuremath{\mathsf{first}}\xspace}
\newcommand{\last}{\ensuremath{\mathsf{last}}\xspace}
\newcommand{\Previouss}[1]{\ensuremath{\Next^{-#1}}\xspace}


% symbol (sub)sets
%TODO use N? CHECK WHAT IS NEEDED
\newcommand{\NCo}{\ensuremath{\Omega}\xspace}%\N_{\mathsf{Co}}}\xspace}
\newcommand{\NPr}[1][]{\ensuremath{\Pi^{#1}}\xspace}%\mathsf{N}_\mathsf{P}^{#1}}\xspace}
\newcommand{\N}{\ensuremath{\mathsf{N}}\xspace}
\newcommand{\NCN}{\ensuremath{\mathsf{N_C'}}\xspace}
\newcommand{\NC}{\ensuremath{\N_{\mathsf{C}}}\xspace}
\newcommand{\NRC}{\ensuremath{\mathsf{N_{RC}}}\xspace}
\newcommand{\NFC}{\ensuremath{\mathsf{N_{FC}}}\xspace}
\newcommand{\NRM}{\ensuremath{\mathbb{R}}\xspace}%{\ensuremath{\mathsf{N}^{-}_{\mathsf{R}}}}\xspace}
\newcommand{\NR}{\ensuremath{\mathsf{N_R}}\xspace}
\newcommand{\NRR}{\ensuremath{\mathsf{N_{RR}}}\xspace}
\newcommand{\NFR}{\ensuremath{\mathsf{N_{FR}}}\xspace}
\newcommand{\NRRM}{\ensuremath{\mathbb{R}_\mathsf{R}}\xspace}%\mathsf{N^{-}_{RR}}}\xspace}
\newcommand{\NFRM}{\ensuremath{\mathbb{R}_\mathsf{F}}\xspace}%\mathsf{N^{-}_{FR}}}\xspace}
\newcommand{\NI}{\ensuremath{\mathsf{N_I}}\xspace}
\newcommand{\NIN}{\ensuremath{\mathsf{N}^{\Nmc}_{\mathsf{I}}}\xspace}
\newcommand{\NIn}{\ensuremath{\mathsf{N_I^n}}\xspace}
\newcommand{\NIR}{\ensuremath{\mathsf{N_I^R}}\xspace}
\newcommand{\NV}{\ensuremath{\mathsf{N_V}}\xspace}
\newcommand{\NFV}{\ensuremath{\mathsf{N_{FV}}}\xspace}
\newcommand{\NT}{\ensuremath{\mathsf{N_T}}\xspace}
\newcommand{\NRRV}{\ensuremath{\mathsf{N_{RRV}}}\xspace}


==> preliminaries-tqa.tex <==





%\section{Introduction to Temporal Conjunctive Query Answering}
%\label{ch:tqa}
%
%We introduce \emph{temporal conjunctive queries}~(TCQs) % as query language, % and the problems we focus on in detail. We 
%%consider a generic DL~\adl, % regard \emph{temporal \QL queries} (TQs) (or \emph{temporal queries}, if \QL is irrelevant or clear from the context); 
%and define the reasoning problems of \emph{TCQ satisfiability} and \emph{TCQ entailment} w.r.t.\ a temporal knowledge base written in a generic DL~\adl.
%% temporal ontology-based data access:
%%\emph{satisfiability of TQs} (investigated in Chapter~\ref{ch:elltl}) and \emph{entailment of TQs} w.r.t.\ a temporal knowledge base written in \adl (studied in Chapters~\ref{ch:eltcqs}, \ref{ch:dlltcqs}, and \ref{ch:exdlltcqs}); 
%%note that \emph{TCQ answering} w.r.t.\ temporal knowledge bases---not necessarily formulated in a description logic---is studied in Chapter~\ref{ch:tqs}.
%%
%%The temporal queries are basically formulas of propositional LTL, but the propositions are replaced by \QL queries;
%%%
%%%\adl axioms and CQs, respectively (i.e., \adl-LTL formulas are also regarded as queries); 
%%and the semantics is suitably lifted from propositional worlds to DL interpretations. 
%%That is, both the \QL queries and the axioms from the temporal knowledge base are interpreted in DL interpretations, and the semantics is based on infinite sequences of such interpretations over the same non-empty domain, called \emph{DL-LTL structures}. %
%%%\footnote{Note
%%
%%In Section~\ref{sec:tqa-tqs}, % and \ref{sec:tqa-elltl}, 
%%we specify the syntax and semantics of the queries and define the problems.  
%A general approach for obtaining containment results for them % problems that 
%which has been proposed in the literature~\cite{BaGL-TOCL12,BaBL-CADE13} is detailed thereafter % in Section~\ref{sec:tqa-on-ubs} 
%since we apply it throughout this work.
%%In Section~\ref{sec:tqa-summary}, w
%We then describe why this approach does not always yield useful containment results for temporal query answering in lightweight description logics and specify problems to solve, our approach, and questions we investigate in this article.
%%In the remainder of the chapter, Section~\ref{sec:tqa-related-work}, we describe related work.
%%Section~\ref{sec:tqa-related-work}, we describe related work.
%%The final summary in Section~\ref{sec:tqa-summary} describes why the previously presented approach does not directly yield useful containment results for temporal query answering in lightweight description logics and---also in view of the related work---specify problems to solve and questions we investigate in the following chapters.
%% and then describe related work (Section~\ref{sec:tqa-related-work}). A general approach for obtaining upper bounds for both problems that has been proposed in literature~\cite{BaGL-TOCL12,BaBL-CADE13} is detailed thereafter, since we apply it throughout this work (Section~\ref{sec:tqa-on-ubs}). In the Summary (Section~\ref{sec:tqa-summary}), we detail why this approach does not directly yield useful containment results for temporal query answering in lightweight description logics and specify the questions we investigate in the following chapters.
%
%%In the following, we focus on a generic DL~\adl and (atemporal) query language~\QL, instantiated later in this chapter; regard \emph{temporal \QL queries} (or \emph{temporal queries} (TQs), if \QL is irrelevant or clear from context); and introduce two kinds of temporal ontology-based data access:
%%\emph{satisfiability of TQs} (investigated in Chapter~\ref{ch:elltl}) and \emph{entailment of TQs} w.r.t.\ a temporal knowledge base written in \adl (studied in Chapters~\ref{ch:eltcqs}, \ref{ch:dlltcqs}, and \ref{ch:exdlltcqs}); note that \emph{temporal query answering} w.r.t.\ temporal knowledge bases---not necessarily formulated in DL---is studied in Chapter~\ref{ch:tqs}.
%%%
%%The queries are basically formulas of propositional LTL, but the propositions are replaced by \QL queries;
%%%
%%%\adl axioms and CQs, respectively (i.e., \adl-LTL formulas are also regarded as queries); 
%%and the semantics is suitably lifted from propositional worlds to Description Logic interpretations. 
%%That is, both the \QL queries and the axioms from the temporal knowledge base are interpreted in DL interpretations, and the semantics is based on infinite sequences of such interpretations over the same non-empty domain, called \emph{DL-LTL structures}. %
%%%\footnote{Note that we employ a semantics that is nowadays standard in the field; ``it is generally
%%	agreed that the semantics of combined temporal description
%%	logics should be based on the Cartesian products of the flow of time \dots and the
%%	domains of the DL interpretations. \dots This
%%	semantics corresponds to the semantics of first-order temporal
%%	logics \dots. In fact, the translation
%%	of standard DLs into first-order logic can be extended
%%	to a translation of temporalised DLs into first-order temporal
%%	logics.''~\cite{AKLWZ-TIME07:temporalising}}
%%\todo{should I switch the 2 above paragraphs?}
%\subsection{Temporal Conjunctive Queries}
%\label{sec:tqa-tqs}
%\index{temporal query|(}
%\emph{Temporal conjunctive queries}\index{temporal conjunctive query|textbf} are a temporal query language introduced in \cite{BaBL-CADE13}. %They represent TQs where \QL is the query language of conjunctive queries.
%\cite{BaBL-CADE13,BaBL-JWS15,BaBL-AI15} investigate the TCQ entailment problem w.r.t.\ temporal knowledge bases in \ALC and other expressive DLs, such as \SHOQ. %Below, we describe how TCQ answering can be reduced to TCQ entailment. We investigate that problem regarding lightweight DLs.%
%%
%TCQs are basically formulas of propositional LTL, but the propositions are replaced by CQs
%%
%%\adl axioms and CQs, respectively (i.e., \adl-LTL formulas are also regarded as queries); 
%and the semantics is suitably lifted from propositional worlds to DL interpretations. 
%That is, both the CQs and the axioms from the temporal knowledge base are interpreted in DL interpretations, and the semantics is based on infinite sequences of such interpretations over the same non-empty domain, called \emph{DL-LTL structures}. %
%%\footnote{Note
%
%%We next specify the temporal query answering setting described in the Introduction. % In particular, the specification is similarly generic,  w
%%Reasoning about TCQs considers \emph{temporal knowledge bases}, which are written in a description logic~\adl. We
%%(i.e., instead of in an arbitrary logic, which is considered in Chapter~\ref{ch:tqs}).
%%In particular, we
%We assume that a subset of the concept and role names is designated as being \emph{rigid}\index{rigid (concept name etc.)|textbf} %\index{concept name!rigid|textbf}\index{role name!rigid|textbf} %\index{rigid symbol}\index{concept name!see also{rigid symbol}}\index{role name!see also{rigid symbol}} 
%(vs.\ \emph{flexible}). %\index{concept name!flexible}\index{role name!flexible}).%
%%\footnote{In the literature, rigid and flexible symbols are also called \emph{global} and \emph{local}, respectively~\cite{AKLWZ-TIME07:temporalising}.}
%%As outlined in Section~\ref{sec:intro-tqa}, t
%The intuition is that the interpretation of rigid names does not change over time. Specifically, the individual names are 
%implicitly assumed to be rigid (i.e., in a DL-LTL structure, an individual name is interpreted by the same domain element at all time points).
%If a concept (axiom) contains only rigid symbols, then we may call it a \emph{rigid} concept (axiom).\todo{check if needed}
%%
%We denote by $\NRC\subseteq\NC$ the rigid concept names, by $\NRR\subseteq\NR$ the rigid role names, and assume a DL %Description Logic 
%signature to be of the form $\adlsignature=(\NI,\NC,\NRC,\NR,\NRR)$\index{signature!DL}, in the following.
%%
%\begin{definition}[DL-LTL structure]\label{def:tqa-tint} 
%	An infinite 
%	sequence $\atint=(\aint_i)_{i\ge0}$ of interpretations $\aint_i=(\Delta,\cdot^{\aint_i})$ for a DL 
%	signature $\adlsignature=(\NI,\NC,\NRC,\NR,\NRR)$ is a  \emph{DL-LTL structure}\index{structure!DL-LTL} if it \emph{respects rigid names}; that is:
%	$\asymbol^{\aint_i}=\asymbol^{\aint_j}\text{ for all } \asymbol\in\NI\cup\NRC\cup\NRR\text{  and }i,j\ge0.$
%	%the following hold, for all $i,j\ge0$:
%	%\begin{itemize}
%	%\item $a^{\aint_i}=a^{\aint_j}$, for all $a\in\NI$;
%	%\item $A^{\aint_i}=A^{\aint_j}$, for all $A\in\NRC$; %and
%	%\item $R^{\aint_i}=R^{\aint_j}$, for all $R\in\NRR$.
%	%\end{itemize}
%%	A DL-LTL structure~$\atint=(\aint_i)_{i\ge0}$ \emph{satisfies}\index{satisfaction!DL axiom} a concept~$C$ at (time point) $i$ if $\aint_i\models C$.
%%	\todo{fix!}
%\end{definition}
%%
%As mentioned above, the interpretations in a DL-LTL structure share one domain (constant domain assumption\index{constant domain assumption}).
%%Further, note that w
%We often do not explicitly mention the signature if it is irrelevant or clear from the context. %, as we keep it for classical interpretations. 
%%
%We may also use this terminology in other settings in that we consider interpretations $\aint_1,\dots,\aint_\ell$ to \emph{respect rigid names} if they agree on the interpretation of all rigid symbols.
%%\todo{better put that in the beginning of the definition?}
%%Subsequently, we introduce the two query languages and problems in detail, provide some auxiliary results, and describe a general approach for obtaining upper bounds for both problems \cite{.}.
%
%Note that we employ a semantics that is nowadays standard in the field \cite[p.~1]{AKLWZ-TIME07:temporalising}. %, as remarked in \cite[p.~1]{AKLWZ-TIME07:temporalising}: %sec 1 , p1
%%\begin{quote}
%%	\textit{``it is generally
%%agreed that the semantics of combined temporal description
%%logics should be based on the Cartesian products of the flow of time (\dots) and the
%%domains of the DL interpretations. (\dots) This
%%semantics corresponds to the semantics of first-order temporal
%%logics (\dots). In fact, the translation
%%of standard DLs into first-order logic can be extended
%%to a translation of temporalised DLs into first-order temporal
%%logics.''}
%%\end{quote}
%Yet, the usual approach of reducing reasoning in the setting with constant domains to reasoning with expanding, decreasing, or varying domains as, for example, detailed in~\cite[\citesec3]{LuWZ-TIME08:survey} does not work for lightweight DLs. In particular, the exact relations between the settings are not clear.
%%Note that we discuss alternative temporal semantics w.r.t.\ applications in the end of Section~\ref{sec:tqs-tqs}.
%\begin{definition}[Syntax of Temporal Knowledge Bases] \label{def:tkb-syntax}
%	A \emph{temporal know\-ledge\index{temporal knowledge base!DL}} \emph{base} (TKB)\index{TKB|see {temporal knowledge base}}
%	$\atkb=\langle\aont,(\afb_i)_{0\le i\le n}\rangle$ consists of an ontology~\aont written in \adl and a non-empty, finite \emph{sequence of ABoxes}\index{sequence!ABoxes|textbf} %$\afb_i$, $i\in[0,n]$, 
%	of \emph{length}\index{length!ABox sequence} $n+1$, where the ABoxes contain only assertions of concept and role names. 
%\end{definition}
%%
%As with atemporal KBs, we assume all concept and role names occurring in some ABox of a TKB to also occur in its ontology.
%%TODO! "contain" not defined for TKB (but O and As)
%%
%We use the notation
%$\NRC(\aont)$ for the set of all rigid concept names that occur in an ontology~\aont, and 
%$\BCr(\aont)$ and $\BCrn(\aont)$ for the restriction of $\BC(\aont)$ and, respectively, $\BCn(\aont)$ to rigid concepts.
%%
%$\Ind(\atkb)$ denotes the set of all individual names occurring in the TKB~\atkb, and 
%$\BC(\afbs)$ and $\NR(\afbs)$ designate the basic concepts and role names in the ABox sequence~\afbs. For simplicity, we sometimes omit the brackets around the ABox sequence.
%
%\begin{definition}[Semantics of Temporal Knowledge Bases] \label{def:tkb-semantics}
%	A DL-LTL structure $\atint=(\aint_i)_{i\ge0}$ over a domain~\adom is a \emph{model}\index{satisfaction (DL)!TKB} of a TKB~$\atkb=\langle\aont,(\afb_i)_{0\le i\le n}\rangle$, written $\atint\models\atkb$, %(vs.\ $\atint\not\models\atkb$), 
%	if the following hold:
%	\begin{itemize}
%		\item $\Imc_i\models\Omc$ for all $i\ge0$,
%		\item $\Imc_i\models\Amc_i$ for all $i\in[0,n]$.
%		%\item \Imf respects rigid names (i.e., $\asymbol^{\Imc_i}=\asymbol^{\Imc_j}$ for all symbols 
%		%$\asymbol\in\NI\cup\NRC\cup\NRR$ and $i, j\ge0$).
%	\end{itemize}
%	%
%	A TKB is \emph{consistent} (or \emph{satisfiable}) if it has a
%	model, and it is \emph{inconsistent} (or \emph{unsatisfiable}) otherwise.
%\end{definition}
%%
%We denote the fact that $\atint\models\atkb$ does not hold by $\atint\not\models\atkb$.
%
%As outlined above, TCQs combine conjunctive queries via LTL operators.
%%
%\begin{definition}[Syntax of Temporal Conjunctive Queries] \label{def:tqs-syntax} 
%	Let $\adlsignature=(\NI,\NC,\NRC,\NR,\NRR)$ be a DL signature.
%	%
%	The set of \emph{temporal conjunctive queries} (TCQs) over \adlsignature is defined by the following grammar:
%	$$\atcq::= \acq\mid 
%	\neg\atcq_1\mid\atcq_1\land\atcq_2\mid
%	\Next\atcq_1\mid\Previous\atcq_1\mid
%	\atcq_1\Until\atcq_2\mid\atcq_1\Since\atcq_2
%	$$
%	where $\acq$ is a CQ over $\adlsignature$, and $\atcq_1$ and $\atcq_2$ are TCQs, in their turn.	
%	
%	A TCQ~\atcq is a \emph{CQ literal}\index{literal}\index{literal!zzza@\igobble |seealso{DL literal}} if it is of the form $(\lnot)\acq$ with \acq being a CQ. It is \emph{positive}\index{positive literal} if $\atcq=\acq$ and otherwise \emph{negative}\index{negative literal}. %The empty conjunction is denoted by \true.
%\end{definition}
%%
%A TCQ~\atcq \emph{contains} a symbol \asymbol  if \asymbol  occurs in \atcq, and
%\atcq \emph{contains} a CQ~\acq if \acq occurs in \atcq at least once not as part of another CQ occurring in \atcq.
%%
%We denote 
%the set of individual names occurring in a TCQ~\atcq by $\Ind(\atcq)$, and the set of variables occurring in~\atcq by $\Var(\atcq)$. %and
%%the set of \emph{free variables}\index{free variable!TCQ} of~\atcq, which is the union of the free variables of all CQs contained in \atcq, by $\FVar(\atcq)$.
%%
%%or \acq has no existentially quantified variables.
%A TCQ~\atcq %is a \emph{CQ literal} if it is of the form $(\lnot)\acq$ with \acq being a CQ, 
%%and it 
%is a \emph{Boolean}\index{Boolean query!TCQ} TCQ if it does not contain non-Boolean CQs. % $\FVar(\atcq) = \emptyset$.
%%
%%the set of variables occurring in~\atcq by $\Var(\atcq)$; and
%%the set of \emph{free}\index{free variable!TQ} variables of~\atcq, which is the union of the free variables of all \QL queries contained in \atcq, by $\FVar(\atcq)$.
%%
%%%or \acq has no existentially quantified variables.
%%A TQ~\atcq %is a \emph{CQ literal} if it is of the form $(\lnot)\acq$ with \acq being a CQ, 
%%%and it 
%%is a \emph{Boolean}\index{Boolean query!TQ} TQ if $\FVar(\atcq) = \emptyset$.
%%%A CQ literal~\atcq based on a CQ~\acq is \emph{positive} if $\atcq=\acq$ and \emph{negative} otherwise. 
%%%In the latter case, the CQ is \emph{negated}.
%%%
%%We assume without loss of generality that the \QL queries contained in a Boolean TQ \atcq use
%%disjoint variables and denote by~\tcqcqs\atcq the set of exactly those \QL queries.%
%%\footnote{If the variables were not disjoint, we could simply rename them. Note that this assumption also applies to Boolean UCQs, which can be considered as TQs where \QL is the language of CQs.}
%%
%%Observe that the definition of TCQs based on CQs is analogous to the definition of propositional LTL formulas based on propositions (see Definition~\ref{def:ltl-syntax}).
%Analogously to LTL, we use abbreviations \true%
%\footnote{For instance, \true may denote a fix TQ $\acq\lor\lnot \acq$, where \acq is an arbitrary \QL query.}\index{true@\true!TQ}
%%
%and \false\index{false@\false!TQ} and may apply derived operators\index{derived operator!TQs} corresponding to those in Figure~\ref{fig:ltl-derived-ops}.
%The empty conjunction and disjunction are interpreted as \true and \false, respectively.
%%\todo{I think this is why I required UCQs to be non-empty. sth does not fit here, right?}
%
%The semantics of TCQs is based on those of CQs.
%%, which we assume to be based on interpretations and to be defined already. 
%%More precisely, we denote the fact that an interpretation~\aint satisfies a \QL query~\acq by $\aint\models\acq$.
%% in the following definition.
%%The semantics of Boolean TQs is given through the notion of homomorphisms \cite{ChMe77:cqsemantics}.%, as it is the case for Boolean CQs.
%%\footnote{
%%	In general, the semantics is based on so-called \emph{certain answers}. These answers are assignments~\aans of the free variables in the given query~\atcqtwo to named individuals occurring in the considered TKB~\atkb so that $\atkb\models\aans(\atcqtwo)$.
%%} 
%%
%\begin{definition}[Semantics of Temporal Conjunctive Queries] \label{def:tcqs-semantics}
%	For a given DL-LTL structure $\atint=(\aint_i)_{i\ge0}$, an $i\ge0$, and a Boolean TCQ~\atcq, the satisfaction relation\index{satisfaction (DL)!Boolean TQ}
%	$\atint,i\models\atcq$ %(vs.\ $\atint,i\not\models\atcq$) 
%	is defined by induction on the structure of~\atcq: for a CQ~\acq, $\atint,i\models\acq$ holds if $\aint_i\models\acq$; for other kinds of TCQs, the corresponding condition of Figure~\ref{fig:ltl-semantics} has to be satisfied. 
%	%
%	\atint is a \emph{model} of \atcq w.r.t.\ a TKB~\atkb if $\atint\models\atkb$.
%%	 and $\atint, n\models\atcq$; and \atint is a \emph{model} of \atcq if it is a model of \atcq w.r.t.\ $\langle\emptyset,\emptyset\rangle$.
%	
%	A Boolean TCQ \atcq is \emph{satisfiable} (w.r.t.\ a TKB~\atkb) if it has a model (w.r.t.\ \atkb); and
%	%
%	\atcq is \emph{entailed}\index{entailment (DL)!Boolean TQ} by a TKB~\atkb, written $\atkb\models\atcq$, if
%	every model of~\atkb is also a model of~\atcq w.r.t.~\atkb.
%	%A mapping $\aans\colon\FVar(\atcq)\to\Ind(\atkb)$, for a TCQ \atcq and TKB \atkb, is a \emph{certain answer} to \atcq w.r.t.\ \atkb if $\atkb\models\aans(\atcq)$, where $\aans(\atcq)$ denotes the Boolean TCQ that is obtained from \atcq by replacing the free variables
%	%according to~\aans.
%\end{definition}
%We denote the fact that $\atint,i\models\atcq$ and $\atkb\models\atcq$ do not hold by $\atint,i\not\models\atcq$ and $\atkb\not\models\atcq$.
%
%%\todo{pull cert out}
%%
%Observe that a model of a TCQ must satisfy the query at the current time point~$n$\index{current time point}, which differs from the corresponding definition for propositional LTL if $n>0$.
%Moreover, for reasoning, we %generally 
%consider TCQs in the context of a TKB.
%%\begin{definition}[Reasoning Problems for TCQs] \label{def:problems-tcqs}
%%For a given Boolean TCQ~\atcq, a TCQ~\atcqtwo, 
%%and a TKB~\atkb, there are the following reasoning problems:\index{reasoning problem!TQ}
%%\begin{itemize}
%%\item 
%%\emph{TCQ Satisfiability:} Is \atcq satisfiable w.r.t.\ \atkb?
%%\index{satisfaction (DL)!TQ} 
%%\item 
%%\emph{TCQ Entailment:}\index{entailment (DL)!Boolean TQ} Does $\atkb\models\atcq$ hold?
%%\item 
%%\emph{TCQ Answering:} Determine all assignments \aans (called \emph{certain answers}\index{certain answer!TCQ}) of the free variables of~\atcqtwo to named individuals occurring in \atkb so that $\akb\models\aans(\atcqtwo)$.
%%
%%%\item 
%%%\emph{TQ Answering}\index{TQ answering}: 
%%%%Compute all certain answers to \atcq w.r.t.\ \atkb.
%%%Determine all assignments \aans (called \emph{certain answers}\index{certain answer}) of the free variables in the query~\atcqtwo to named individuals occurring in \atkb so that $\akb\models\aans(\atcqtwo)$.
%%\end{itemize}
%%\end{definition}
%%
%%\item 
%%\emph{TQ Answering}\index{TQ answering}: 
%%%Compute all certain answers to \atcq w.r.t.\ \atkb.
%%Determine all assignments \aans (called \emph{certain answers}\index{certain answer}) of the free variables in the query~\atcqtwo to named individuals occurring in \atkb so that $\akb\models\aans(\atcqtwo)$.
%%
%%As it is the case for UCQs, the set of certain answers to a Boolean TQ is $\{() \}$ (``true'') if $\atkb\models\atcq$ and $\emptyset$ (``false''), otherwise. 
%%Query answering for Boolean queries thus represents a decision problem, the query entailment problem. The problem of finding all answers to a possibly non-Boolean query is known as query answering. Although it is not necessarily efficient in practice, the problem of answering a TQ~\atcq w.r.t.\ a TKB~\atkb can easily be reduced to TQ entailment, by considering exponentially many entailment problems for the $|\NI(\atkb)|^{|\FVar(\atcq)|}$ possible certain answers that are to be considered.
%%
%We often solve the entailment problem by reducing it to the satisfiability problem: If $\lnot\atcq$ is satisfiable, then $\atcq$ is not entailed.
%%
%%As it is the case for UCQs, the set of certain answers to a Boolean TCQ is $\{() \}$ (``true'') if $\atkb\models\atcq$ and $\emptyset$ (``false'') otherwise. 
%%Query answering for Boolean TCQs thus represents the decision problem of query entailment. 
%%This is why we focus on Boolean TCQs in Chapters~\ref{ch:eltcqs}--\ref{ch:exdlltcqs}. 
%%%The problem of finding all answers to a possibly non-Boolean query is known as query answering. 
%%Although answering non-Boolean queries is not necessarily efficient in practice, the problem of answering a TCQ~\atcq w.r.t.\ a TKB~\atkb can easily be reduced to TCQ entailment, by considering exponentially many entailment problems for the $|\NI(\atkb)|^{|\FVar(\atcq)|}$ possible certain answers that are to be considered.
%
%
%\todo{detail relationship to query ansering?; assume TCQs to be boolean?}
%The technical assumptions we make about TCQs are as follows. 
%We assume without loss of generality that the CQs contained in a Boolean TCQ \atcq use
%disjoint variables and denote by~\tcqcqs\atcq the set of exactly those CQs.%
%\footnote{If the variables were not disjoint, we could simply rename them. Note that this assumption also applies to Boolean UCQs.}
%%
%We further assume that TCQs contain only individual names that occur in the ABoxes, and only concept and role names that occur in the ontology; this is clearly without loss of generality, especially because of the assumption that all concept and role names occurring in a TKB occur in its ontology.
%%
%For simplicity, we assume all Boolean CQs contained in TCQs to be connected in the following; note that this assumption thus also applies to all (U)CQs we regard since they are also TCQs.
%To see that this is without loss of generality, 
%consider a Boolean TCQ \atcq containing a CQ \acq that is not connected. In that case, \acq can be replaced by a conjunction $\acq_1 \land\dots\land\acq_\ell$ of CQs $\acq_1 ,\dots,\acq_\ell$ that represent a partition of \acq.
%%	$\toqgraph{\acq_1},\dots,\toqgraph{\acq_\ell}$ are the connected components of $\toqgraph\acq$. 
%This conjunction is of linear size in the size of \acq and the resulting TCQ has exactly the same models as \atcq. More precisely, every homomorphism of \acq into an interpretation~\aint is also a homomorphism of, respectively, $\acq_1,\ldots, \acq_\ell$ into \aint if it is restricted to the corresponding terms. And, because of the disjointness of $\term(\acq_1),\dots,\term(\acq_\ell)$, given by the definition of a partition, %, which is given by the fact that we consider the connected components of $\toqgraph\acq$, 
%every collection of homomorphisms of $\acq_1,\ldots, \acq_\ell$ into an interpretation~\aint can be unified to a homomorphism of $\acq$ into \aint. 
%
%
%%
%%We therefore focus on satisfiability and entailment in this work.
%
%According to \cite{BaBL-JWS15}, 
%the entailment problem of a TCQ~\atcq w.r.t.\ a TKB $\langle\aont,(\afb_i)_{0\le i\le n}\rangle$ can be solved by considering an extension of~\atcq w.r.t.\ $\langle\aont,\emptyset\rangle$---regarding the trivial sequence of ABoxes. 
%%\footnote{The temporal query language considered in \cite{BaBL-JWS15} is that of temporal conjunctive queries, but the result is independent of the \QL queries and hence extends to our setting.}
%Note that this sometimes eases analysis but is not useful if data complexity is considered, because the data is incorporated into the query. 
%%This is done by rewriting the Boolean TCQ~$\phi$ into a Boolean TCQ~$\phi'$ of 
%%polynomial size in the size of $\phi$ and the TKB \Omc such that answering
%%$\phi$ at time point $n$ is equivalent to answering $\phi'$ at time point $0$
%%w.r.t.\ the trivial sequence of ABoxes.
%%%
%%However, this obviously does not work for data complexity, as the resulting
%%TCQ is no longer independent of the data.
%%
%\begin{rwlemma}[{{\cite[\citelem6.1]{BaBL-JWS15}}}]
%	\label{prop:tcqs-encode-aboxes}
%%	Let \QL be such that every assertion represents a \QL query.
%	For every TKB~$\atkb=\langle\aont,(\afb_i)_{0\le i\le n}\rangle$ and Boolean TCQ~\atcq, there is a Boolean TCQ $\atcq'$ of size polynomial in the 
%	size of \atcq and \atkb such that $\atkb\models\atcq$ iff 
%	$\langle\aont,\emptyset\rangle\models\atcq'$.
%\end{rwlemma}
%\todo{remove as a lemma? or `convert' to a fact?}
%
%We often regard TCQs~\atcq that do not contain temporal operators; for example, UCQs or conjunctions of CQ literals.
%It can be readily checked that the satisfaction of \atcq by a DL-LTL structure $\atint= (\aint_i)_{i\ge0}$ at time point 
%$i$ then only depends on the interpretation $\aint_i$, according to the definition and the conditions in Figure~\ref{fig:ltl-semantics}. For simplicity, we then often write $\aint_i\models\atcq$ instead of $\atint,i\models\atcq$. 
%%
%In this context, it is also sufficient to consider classical knowledge bases\index{classical knowledge base|see{knowledge base}}~$\langle\aont,\afb\rangle$, which can be regarded as TKBs with a single ABox.
%
%Since TCQs can be related to propositional LTL formulas in an intuitive way, by abstracting from the CQs, we can analyze the temporal structure of the TCQ separately from the DL part.
%%
%\begin{definition}[Propositional Abstraction] \label{def:tcqs-pa}\label{def:elltl-pa}
%Let \atcq be a TCQ and $\apropset_\atcq$ be a finite set of propositional variables so that there is a bijection~$\pa\cdot$ mapping the CQs contained in \atcq to elements of~$\apropset_\atcq$.%
%\footnote{Note that such a set $\apropset_\atcq$ and bijection $\pa\cdot$ obviously exist for every TCQ~\atcq.}
%%
%The \emph{propositional abstraction}\index{propositional abstraction}~$\pa\atcq$ of \atcq w.r.t.\ $\pa\cdot$ is the propositional LTL formula obtained from \atcq by replacing every CQ~\acq in \atcq by~$\pa\acq$.
%
%The \emph{propositional abstraction}~$\pa\atint$ of a DL-LTL structure $\atint=(\aint_i)_{i\ge0}$ w.r.t.\ $\pa\cdot$ is the propositional LTL structure $\pa\atint=(w_i)_{i\ge0}$ where, for all $i\ge0$, \[w_i:=\{ \pa\acq\mid\text{\acq is contained in \atcq},\ \aint_i\models\acq \}.\]
%\end{definition}
%%
%% Again for simplicity, for a sub-TCQ ψ of φ, we denote by ψp the propositional abstraction of ψ w.r.t. the restriction of p to CQ(ψ). 
%%The propositional abstraction φp of φ w.r.t. p is a propositional LTL-formula that allows us to analyse the temporal structure of φ separately from the CQ-component. The following lemma is very similar to Lemma 3.8, and its proof is analogous.
%%
%This abstraction obviously retains the semantics.
%That is, for a DL-LTL structure~\atint that is a model of a TKB \atkb and  a bijection~$\pa\cdot$ as in Definition~\ref{def:tcqs-pa}, we have:
%\atint is a model of a TCQ \atcq w.r.t.\ \atkb iff $\pa{\atint}$ is a model of~$\pa{\atcq}$.
%%
%%%
%%\begin{fact}%[{{\cite[Lemma 5.14]{phdmarcel}}}]
%%Let \atint be a DL-LTL structure that is a model of a TKB \atkb and $\pa\cdot$ be a bijection as in Definition~\ref{def:tcqs-pa}.
%%Then, \atint is a model of a TQ \atcq w.r.t.\ \atkb iff $\pa{\atint}$ is a model of~$\pa{\atcq}$.
%%\end{fact}
%
%%In the remainder of the section, we present the two instantiations of TQs this work focuses on: temporalized DL axioms (investigated in Chapter~\ref{ch:elltl}) and temporal conjunctive queries (investigated in Chapters~\ref{ch:eltcqs} to~\ref{ch:exdlltcqs}).
%%Notes that, in Chapter~\ref{ch:tqs}, we consider various other instantiations.
%
%%\subsection*{Temporalized Description Logic Axioms}
%%%	The Temporal Description Logic \EL-LTL}
%%\label{sec:tqa-elltl}\index{el-ltl@\EL-LTL|see{\adl-LTL}}\index{dl-lite-ltl@\DLLite-LTL|see{\adl-LTL}}\index{alc-ltl@\ALC-LTL|see{\adl-LTL}}
%%%\todo{for el ltlt say before what are global gcis}
%%As it has been done for \textit{TDL-Lite}~\cite{AKLWZ-TIME07:temporalising}, \DLLite logics that allow for temporal operators in concept expressions; \ALC~\cite{BaGL-TOCL12}; and \SHOQ~\cite{phdmarcel}; we combine the operators of LTL with \adl axioms into the temporal query language \adl-LTL\index{DL-ltl@\adl-LTL}.%
%%\footnote{Note that the queries in the related works do not contain past operators.
%%	}
%% That is, DL axioms are considered to be the \QL queries. We specifically regard lightweight DLs~\adl and investigate the satisfiability problem. 
%%
%%In particular, we disregard TKBs by assuming them to be empty---which means that we always have $n=0$. 
%%Observe that \adl-LTL then represents a kind of temporal DL, and TQs are also called \emph{\adl-LTL formulas}\index{formula!DL-ltl@\adl-LTL}.
%%Nevertheless, there are close connections to the general setting.
%%\begin{example}\label{ex:tqa-ggci-tkb-relation}
%%	The question if an \adl TKB $\langle\aont,(\afb_i)_{0\le i\le n}\rangle$ is consistent can also be decided by asking if the following \adl-LTL formula is satisfiable (see also \rwlem\ref{prop:tcqs-encode-aboxes}):
%%	\[\Boxf(\bigwedge\aont)\land \bigwedge_{\substack{0\le i\le n,\\\aaxiom\in\afb_i}}\Next^i\aaxiom.\]
%%	%$\Next^i$ denotes a sequence of $i$ $\Next$ operators.
%%\end{example}
%%Observe that the formula in the example is of special shape because it does not contain arbitrary combinations of CIs, but only a conjunction prefixed by $\Boxf$. This is known as \adl-LTL with \emph{global CIs}\index{global CI} (vs.\ \emph{local}\index{local CI} CIs) and investigated separately in this work.
%%%In this section, we thus consider \EL as a concrete Description logic.
%%
%%Lastly, note that we generally use the notion \emph{\adl literals}\index{DL literal}\index{DL literal!zzza@\igobble |seealso{literal}} for the literals mentioned in Definition~\ref{def:tqs-tqs-syntax} if \QL is the language of \adl axioms.
%
%%\subsection*{Temporal Conjunctive Queries}
%%\label{sec:tqa-tcqs}
%%
%%\emph{Temporal conjunctive queries}\index{temporal conjunctive query|textbf} (TCQs) are a temporal query language introduced in \cite{BaBL-CADE13}. They represent TQs where \QL is the query language of conjunctive queries.
%%\cite{BaBL-CADE13,BaBL-JWS15,BaBL-AI15} investigate the TCQ entailment problem w.r.t.\ temporal knowledge bases in \ALC and other expressive DLs, such as \SHOQ. Below, we describe how TCQ answering can be reduced to TCQ entailment. We investigate that problem regarding lightweight DLs.
%%
%%We next introduce additional syntax, describe the relation between TCQ entailment and TCQ answering, and provide technical assumptions we make about TCQs throughout this thesis. 
%%
%%For a TCQ~\atcq, we denote the set of variables occurring in~\atcq by $\Var(\atcq)$; and
%%the set of \emph{free variables}\index{free variable!TCQ} of~\atcq, which is the union of the free variables of all CQs contained in \atcq, by $\FVar(\atcq)$.
%%%
%%%or \acq has no existentially quantified variables.
%%A TCQ~\atcq %is a \emph{CQ literal} if it is of the form $(\lnot)\acq$ with \acq being a CQ, 
%%%and it 
%%is a \emph{Boolean}\index{Boolean query!TCQ} TCQ if $\FVar(\atcq) = \emptyset$.
%%A CQ literal~\atcq based on a CQ~\acq is \emph{positive} if $\atcq=\acq$ and \emph{negative} otherwise. 
%%In the latter case, the CQ is \emph{negated}.
%
%%For determining complexity, we have to focus on a decision problem. The focus of research therefore is usually on query entailment instead of on query answering.
%%\begin{definition}[TCQ Answering]
%%For a given TCQ~\atcq, 
%%the problem of \emph{TCQ Answering}\index{query answering!TCQ}  is defined as follows:
%%%Compute all certain answers to \atcq w.r.t.\ \atkb.
%%Determine all assignments \aans (called \emph{certain answers}\index{certain answer!TCQ}) of the free variables of~\atcq to named individuals occurring in \atkb so that $\akb\models\aans(\atcq)$.
%%\end{definition}
%%
%%
%%As it is the case for UCQs, the set of certain answers to a Boolean TCQ is $\{() \}$ (``true'') if $\atkb\models\atcq$ and $\emptyset$ (``false'') otherwise. 
%%Query answering for Boolean TCQs thus represents the decision problem of query entailment. 
%%This is why we focus on Boolean TCQs in Chapters~\ref{ch:eltcqs}--\ref{ch:exdlltcqs}. 
%%%The problem of finding all answers to a possibly non-Boolean query is known as query answering. 
%%Although answering non-Boolean queries is not necessarily efficient in practice, the problem of answering a TCQ~\atcq w.r.t.\ a TKB~\atkb can easily be reduced to TCQ entailment, by considering exponentially many entailment problems for the $|\NI(\atkb)|^{|\FVar(\atcq)|}$ possible certain answers that are to be considered.
%%
%%
%%The technical assumptions we make about TCQs are as follows. 
%%We assume without loss of generality that the CQs contained in a Boolean TCQ \atcq use
%%disjoint variables and denote by~\tcqcqs\atcq the set of exactly those CQs.%
%%\footnote{If the variables were not disjoint, we could simply rename them. Note that this assumption also applies to Boolean UCQs.}
%%%
%%We further assume that TCQs contain only individual names that occur in the ABoxes, and only concept and role names that occur in the ontology; this is clearly without loss of generality, especially because of the assumption that all concept and role names occurring in a TKB occur in its ontology.
%%%
%%For simplicity, we assume all Boolean CQs contained in TCQs to be connected in the following; note that this assumption thus also applies to all (U)CQs we regard since they are also TCQs.
%%To see that this is without loss of generality, 
%%consider a Boolean TCQ \atcq containing a CQ \acq that is not connected. In that case, \acq can be replaced by a conjunction $\acq_1 \land\dots\land\acq_\ell$ of CQs $\acq_1 ,\dots,\acq_\ell$ that represent a partition of \acq.
%%%	$\toqgraph{\acq_1},\dots,\toqgraph{\acq_\ell}$ are the connected components of $\toqgraph\acq$. 
%%This conjunction is of linear size in the size of \acq and the resulting TCQ has exactly the same models as \atcq. More precisely, every homomorphism of \acq into an interpretation~\aint is also a homomorphism of, respectively, $\acq_1,\ldots, \acq_\ell$ into \aint if it is restricted to the corresponding terms. And, because of the disjointness of $\term(\acq_1),\dots,\term(\acq_\ell)$, given by the definition of a partition, %, which is given by the fact that we consider the connected components of $\toqgraph\acq$, 
%%every collection of homomorphisms of $\acq_1,\ldots, \acq_\ell$ into an interpretation~\aint can be unified to a homomorphism of $\acq$ into \aint. 
%
%
%
%
%
%
%\index{temporal query|)}
%\subsection{A General Approach for Solving Satisfiability}
%\label{sec:tqa-on-ubs}


%\subsection{Problem Analysis and Contributions} %Problem Analysis and 
%\label{sec:tqa-summary}

%We focus on the temporal query languages and reasoning problems %---satisfiability, entailment, and query answering---
%introduced in this chapter. 
%We study TCQ entailment regarding various different settings:
%\begin{itemize}
%\item We consider \EL and different \DLLite fragments as instantiations of~\adl. %as ontology languages. 
%\item We consider different settings w.r.t.\ the rigid symbols and distinguish if no rigid names, only rigid concept names, or both rigid concept and role names are allowed.
%\item We investigate both combined and data complexity.
%\end{itemize}
%For solving satisfiability, % and entailment, 
%We generally solve entailment based on the approach presented in Section~\ref{sec:tqa} %(see \rwlem\ref{prop:tcq-sat-iff}) 
%and, for deciding the TCQ satisfiability problem, focus on the three 
%problems of:
%\begin{enumerate}[label=\textnormal{(\roman*)}]
%	\item\label{def:tqa-task-obtaining} 
%	obtaining \as and $\iota$,
%	\item\label{def:tqa-task-ltl} 
%	solving the LTL satisfiability test (t-satisfiability), and
%	\item\label{def:tqa-task-dl}  solving the DL satisfiability test(s) (r-satisfiability). %
%%	\footnote{We use the notation of Section~\ref{sec:tqa-on-ubs}.}
%	\end{enumerate}
%%
%%Observe the following.
%%
%%
%Regarding the choice of methods to obtain \as and $\iota$ for~\ref{def:tqa-task-obtaining}, we have that each can be obtained by enumeration, guessing, or direct construction, depending on the complexity class we target.
%The size of \as is exponential in that of the considered TCQ~\atcq, and the size of the mapping $\iota$ is linear in $n$, but there are exponentially many possible such mappings.
%Note that, in the special case where we have the trivial ABox sequence~$(\emptyset)_{0\le i\le n}$, a mapping $\iota$ can always be obtained easily if there is a set~\as that satisfies all but the last conditions of t-satisfiability and r-satisfiability, respectively.
%To see this, observe that \as must not be empty, and that the last condition in Definition~\ref{def:tqa-r-sat} requires the world $\ax_{\iota(0)}$, an element of $\as$, to be consistent w.r.t.\ the KB $\langle\aont,\emptyset\rangle$, 
%which is true for every world in \as if \as satisfies the other conditions in that definition. Given that the other conditions are met, the last condition in Definition~\ref{def:tqa-t-sat} can thus easily be satisfied by defining $\iota\colon [0,0]\to[1,k]$ such that it maps $0$ to the index of the world from \as that exists because of the first condition. %We state that as a fact for future reference.
%%
%%We hence do not have to consider that condition for our characterization and can disregard $\iota$. % w.r.t.\ the r-satisfiability test.
%\begin{fact}\label{fact:tqa-iota-emptyaboxes}
%%A TQ is satisfiable w.r.t.\ a TKB~$\langle\aont,(\emptyset)_{0\le i\le n}\rangle$ if
%%there is a set~\as 
%%that satisfies all but the last conditions in Definitions~\ref{def:tqa-t-sat} and \ref{def:tqa-r-sat}.
%For a TCQ~\atcq, TKB~$\langle\aont,(\emptyset)_{0\le i\le n}\rangle$, and set~\as 
%that satisfies all but the last conditions in Definitions~\ref{def:tqa-r-sat} and \ref{def:tqa-t-sat}, there exists a mapping $\iota\colon [0,n]\to[1,k]$ so that the remaining conditions are also satisfied.
%%the mapping $\iota\colon [0,0]\to[1,k]$ with $\iota(0)=i$ 
%%For a TCQ~\atcq, the TKB~$\langle\aont,(\emptyset)_{0\le i\le n}\rangle$, and a set~\as 
%%that satisfies all but the last conditions in Definitions~\ref{def:tqa-r-sat} and \ref{def:tqa-t-sat}, we have $\atkb\$.
%%%assuming we have $w_0=W_i$ w.r.t.\ the latter,
%%the mapping $\iota\colon [0,0]\to[1,k]$ with $\iota(0)=i$ 
%\end{fact}
%
%Problem~\ref{def:tqa-task-ltl} is independent of the DL. Moreover, it can be solved in exponential time w.r.t.\ combined complexity and in polynomial time w.r.t.\ data complexity, by using a reduction to the emptiness of a B\"uchi automaton~\cite[\citelem4.12]{BaBL-JWS15}.
%
%Regarding Problem~\ref{def:tqa-task-dl}, we have two characterizations of r-satisfiability, Definition~\ref{def:tqa-r-sat} and \rwlem\ref{prop:tcq-r-sat-iff}.
%The critical point with the former is the requirement that the interpretations %exponentially many models 
%$\Jmc_1,\dots, \Jmc_k,\Imc_0,\dots, \Imc_n$ 
%share a common domain, % (i.e., the number $k$ is exponential in $\atcq$). 
%because the satisfiability tests for different interpretations cannot be done independently of each other, if rigid symbols are considered.
%%$k$ is exponential in the size of \atcq.
%%as in Definition~\ref{def:tqa-r-sat}. But we adapt the first condition in that we assume the domains of the interpretations to be disjoint w.r.t.\ the unnamed individuals and use the additional data together with specific conditions to take over the functions of the shared domain. It turned out 
%Observe that $\Jmc_1,\dots, \Jmc_k$ characterize the satisfiability of the  conjunctions $\chi_i$ w.r.t.\ $\langle\aont,\emptyset\rangle$, $i\in[1,k]$, respectively. Moreover, the functions of the common domain are mainly two, which gets more evident if the additionally required respect of rigid symbols is considered: 
%\begin{enumerate}[label=\textnormal{(F\arabic*)}]
%\item\label{eq:tqa-domfunctinds} Synchronize the interpretation of rigid names w.r.t.\ the named individuals.
%\item\label{eq:tqa-domfunctchis} Guarantee that the satisfiability of the conjunctions $\chi_i$, $i\in[1,k]$, which is represented by the respective interpretation $\Jmc_i$, is not contradicted by the interpretation of the rigid names in the other interpretations.
%\end{enumerate}
%%
%Problem~\ref{def:tqa-task-dl} thus depends on % \QL and 
%\adl, and especially on which symbols are allowed to be rigid. 
%%
%This can be similarly seen by considering \rwlem\ref{prop:tcq-r-sat-iff}. If rigid names are not considered, then the $k$ conjunctions $\chi^{(i)}$ with $i\in[1,k]$ in the conjunction $\chi_{\as,\iota}$ do not share any symbols. That is, their satisfiability can be tested independently of each other. This is important considering the fact that the size of $\chi_{\as,\iota}$ depends on the exponential number $k$. 
%\begin{rwlemma}[{{\cite[\citelem5.1]{BaGL-TOCL12}}}]
%	\label{prop:tqa-worigid-ws-independent}
%	Let $\chi_1,\dots,\chi_\ell$ be conjunctions of CQ literals, $\aont_1,\dots,\aont_\ell$ be ontologies, and $\Amc_1,\dots,\Amc_\ell$ be ABoxes so that elements with different index $i\in[1,\ell]$ do not share concept and role names.
%	Then the conjunction $\chi_1\land\dots\land \chi_\ell$ is satisfiable w.r.t.\ the KB~$\langle\bigcup_{1\le i\le \ell}\aont_{i},\bigcup_{1\le i\le \ell}\afb_i\rangle$ iff, for each $i\in[1,\ell]$, $\chi_i$ is satisfiable w.r.t.\ $\langle\aont_{i},\afb_i\rangle$.
%\end{rwlemma}
%Again, \cite[\citelem5.1]{BaGL-TOCL12} refers to a slightly different temporal query language, % \QL of \ALC axioms, 
%but the result also holds in our setting.
%
%%
%%The following fact is then easy to verify.
%%\todo{or is that polynomial in the data?}
%%%
%%\begin{rwlemma}\label{prop:tqa-r-sat-wo-rigid}
%%Let \NRC and \NRR be empty.
%%If the satisfiability problem for conjunctions of \QL query literals w.r.t.\ an \adl-KB is contained in a class $C$, % \supseteq\ExpTime$ ($C\supseteq\PTime$) 
%%w.r.t.\ combined (data) complexity, then the r-satisfiability problem w.r.t.\ an arbitrary mapping~$\iota$ and \adl-KB is so as well if $C\supseteq\ExpTime$ ($C\supseteq\PTime$), and otherwise in $\ExpTime$ ($\PTime$).\qed
%%\end{rwlemma}
%%
%Rigid names, on the other hand, generally require the consideration of the whole conjunction. We thus get only rather high upper bounds from \rwlem\ref{prop:tcq-r-sat-iff}.
%%
%\begin{lemma}\label{lem:tqa-tq-sat-containment}
%%Let \QL be such that every assertion in \adl is a \QL query.
%If the satisfiability problem for conjunctions of CQ literals w.r.t.\ a \adl KB is contained in \NP, %a complexity class $C\supseteq\NExpTime$ $C\supseteq\NP$ 
%%w.r.t.\ combined (data) complexity, 
%then 
%the satisfiability problem for TCQs w.r.t.\ a \adl TKB is contained in \NExpTime (\NP), and the entailment problem is contained in \coNExpTime (\coNP), w.r.t.\ combined (data) complexity. %$C$ or its complementary complexity class, depending on whether $C$ is deterministic or not.
%\end{lemma}
%\begin{proof}
%We focus on the satisfiability problem and regard the conditions in \rwlem\ref{prop:tcq-sat-iff}.
%Given the above observations, \ref{def:tqa-task-obtaining}~both the set~$\as\subseteq 2^\pv$ of worlds and the mapping~$\iota\colon[0,n]\to[1,k]$ can be nondeterministically guessed in exponential (polynomial) time, and \ref{def:tqa-task-ltl}~t-satisfiability can be decided in exponential (polynomial) time in the input (data). Regarding \ref{def:tqa-task-dl}~r-satisfiability, we have that
%$\chi_{\as,\iota}$ is of size exponential in $|\atcq|$ because of the first $k$ conjuncts.
%%, and polynomial in \atkb, and the size of $\aont_{\as,\iota}$ is linear in that of \aont and exponential in that of~\atcq. 
%The size of each of the other $n$ conjuncts %~$\chi^{(k+i+1)}$, $i\in[0,n]$, 
%is $\log(n)$ times (i.e., for the representation of the index) the sum of a number linear in $|\atcq|$, for the conjuncts~$\chi^{(k+i+1)}$, $i\in[0,n]$. %and  $|\afb_i|$, for the respective ABox~$\afb_i$. %; times , for the representation of the index.
%The size of $\aont_{\as,\iota}$ is exponential in $|\atcq|$, and linear in $|\aont|$ and $n$. The size of \afb is $\log(n)$ times the sum of all $|\afb_i|$, $i\in[1,n]$, and thus polynomial in the data.
%Given the assumption (and the fact that $|\atcq|$ and $|\aont|$ are constants), the satisfiability of the conjunction in \rwlem\ref{prop:tcq-r-sat-iff} can be tested in nondeterministic exponential (polynomial) time.
%%
%TCQ satisfiability is thus contained in \NExpTime (\NP), and entailment in \coNExpTime (\coNP).
%\end{proof}
%%The size of the first $k$ conjuncts of $\chi^{(i)}$, $i\in[1,k]$, is constant since they do not depend on the input ABoxes.
%%%
%%The size of each conjunct $\chi^{(k+i+1)}$, $i\in[0,n]$, is the sum of $|\afb_i|$, where $\afb_i$ is the respective ABox, and a constant factor.
%%%
%%The size of $\aont_{\as,\iota}$ is linear in~$n$.
%
%
%The above observations show that, in many cases, we cannot directly follow the approach of \cite{BaGL-TOCL12,BaBL-JWS15} because we target considerably lower complexity results. While the size of $\iota$ is only an obstacle for designing algorithms of sublinear complexity, the exponential size of \as makes it impossible to guess (and store) this set by using only a polynomial amount of space.
%And known results only allow to solve Problems~\ref{def:tqa-task-ltl} and \ref{def:tqa-task-dl} in exponential time. 
%The trivial approach of \rwlem\ref{prop:tcq-sat-iff} does hence neither provide an upper bound of \PSpace w.r.t.\ combined complexity, the lower bound we have from LTL satisfiability,
%nor tractable data complexity, if rigid symbols are considered.
%Yet, for the Horn fragments of \DLLite, we usually have such reasoning complexities. Indeed, we obtain such \PSpace and tractability results. 

\subsection{A Polynomial-Space Algorithm}


%, even in some settings with rigid symbols. %To this end, we develop a new approach based on adapting the algorithm originally proposed for solving the LTL satisfiability problem (see Algorithm~\ref{algo:ltl-sat}).
%
%\todo{$s\ge n$ also works right? instead of $>$}
%\begin{algorithm}
%	\KwIn{TQ~\atcq, TKB~$\langle\aont,(\afb_i)_{0\le i\le n}\rangle$}
%	\KwOut{\true if \atcq is satisfiable, otherwise \false}
%	\BlankLine
%	Do some \textbf{preprocessing}\;\colorbox{mygray}{{\algofont{\algoBoolCons}}}
%	Guess an \textbf{r-complete tuple} of size polynomial in $|\atcq|$\;
%	$i:=0$\;
%	$s:=$ Guess a number exponential in $|\pa\atcq|$ and \textbf{so that $s\ge n$}\;
%	$p:=$ Guess a number exponential in $|\pa\atcq|$\;
%	\BlankLine
%$\Fmc_{\fnext}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
%$\Fmc_{\fs}:=\emptyset$, %\;
%$\Fmc_{\Until}:=\emptyset$\;
%%
%\BlankLine
%$\Fmc_{\fnow}:=$ Guess a set of subformulas of \altlform\;
%\BlankLine
%\If{\textbf{not} \textnormal{{\algofont{\algoBoolCons}}($\Fmc_{\fnow}$) \textbf{or} 
%		\textbf{\itshape not} \textnormal{{\algofont{\algoInitial}}($\Fmc_{\fnow}$, $\altlform$)}
%	}
%}{return \false}
%%$\Fmc_{\fnow}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
%%$\Fmc_{\fs}:=\emptyset$, %\;
%%$\Fmc_{\Until}:=\emptyset$\;
%%%
%%\BlankLine
%%$\Fmc_{\fnext}:=$ Guess a set of subformulas of \altlform\;
%%\BlankLine
%%\If{\textbf{not} \textnormal{\algofont{\algoBoolCons}($\Fmc_{\fnext}$) \textbf{or} 
%%		\textbf{\itshape not} \textnormal{\algofont{\algoInitial}($\Fmc_{\fnext}$, $\altlform$)} \textbf{or} 
%%		$\altlform\not\in\Fmc_{\fnext}$  
%%	}
%%}{return false}
%\BlankLine
%\While{$i\le s+p$}{\BlankLine
%		Update $\Fmc_{\fnow}$ and $\Fmc_{\fnext}$ and
%		proceed as in Algorithm~\ref{algo:ltl-sat} for input $\pa\atcq$, Lines~9 to~15\;
%	\BlankLine
%	\lIf{$i=n$ \textbf{and} $\pa\atcq\not\in\Fmc_{\fnow}$}{return \false}
%	\BlankLine
%	$\ax:=\Fmc_{\fnow}\cap\pv$\;\BlankLine
%%	$\overline{\ax}:=\pv\setminus\Fmc_{c}$\;
%	\lIf{$i>n$}{$\Amc_i:=\emptyset$}\BlankLine
%%	Initialize \textbf{additional parameters}\;
%
%	\If{\textnormal{one of the \textbf{r-Satisfiability tests} fails}}{return \false}
%%	$r:=$ \false if one of the \textbf{r-Satisfiability tests} fails, otherwise \true\;
%%	\lIf{$r=$ \false}{return false}
%	\BlankLine
%	$i:=i+1$\;
%%	Continue as in the loop of Algorithm~\ref{algo:ltl-sat}, Line~13\;
%%	\lIf{$i=s$}{$\Fmc_s:=\Fmc_c$}
%%	\BlankLine
%%	\If{$i\ge s$}{
%%		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_{\Until}\cup\Fmc_{c}$ so that $\altlform_2\not\in \Fmc_{c}$\;
%%	}
%}
%Continue as in Algorithm~\ref{algo:ltl-sat}, Line~17
%%\If{$\Fmc_{\Until}=\emptyset$ \textbf{and} \textnormal{\algofont{\algoTCons}($\Fmc_{\fnow}$, $\Fmc_{s}$)}
%%}{
%%return \true}
%%return \false
%
%\caption{Procedure for Deciding TQ Satisfiability}
%\label{algo:tq-sat}
%\end{algorithm}
%\begin{algorithm}[tb]
%\KwIn{TCQ~\atcq, TKB~$\atkb~\langle\aont,(\afb_i)_{0\le i\le n}\rangle$}
%\KwOut{\true if \atcq is satisfiable w.r.t.\ \atkb, otherwise \false}
%\BlankLine
%%$\atcq:=$ 
%%\colorbox{AlgoGray}{\algofont{\algoPreprocessing}(\atcq)}\;
%$d:=$ \colorbox{AlgoGray}{\algofont{\algoGuessing}($\atcq, \atkb$)}\;
%%Guess an \textbf{r-complete tuple} of size polynomial in $|\atcq|$\;
%$i:=0$\;
%$s:=$ Guess a number $\le2^{|\pa\atcq|}$, $>0$, and \colorbox{AlgoGray}{such that $s\ge n$}\;
%$p:=$ Guess a number $\le4^{|\pa\atcq|}$\;
%\BlankLine
%$\Fmc_{\fnext}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
%$\Fmc_{\fs}:=\emptyset$, %\;
%$\Fmc_{\Until}:=\emptyset$\;
%%
%\BlankLine
%$\Fmc_{\fnow}:=$ Guess a subset of $\Clo(\{\pa\atcq \})$\;
%\BlankLine
%\If{\textbf{not} \textnormal{{\algofont{\algoBoolCons}}($\Fmc_{\fnow}$) \textbf{or} 
%		\textbf{\itshape not} \textnormal{{\algofont{\algoInitial}}($\Fmc_{\fnow}$%, $\altlform$
%			)} 
%	}
%}{return \false}
%%$\Fmc_{\fnow}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
%%$\Fmc_{\fs}:=\emptyset$, %\;
%%$\Fmc_{\Until}:=\emptyset$\;
%%%
%%\BlankLine
%%$\Fmc_{\fnext}:=$ Guess a set of subformulas of \altlform\;
%%\BlankLine
%%\If{\textbf{not} \textnormal{\algofont{\algoBoolCons}($\Fmc_{\fnext}$) \textbf{or} 
%%		\textbf{\itshape not} \textnormal{\algofont{\algoInitial}($\Fmc_{\fnext}$, $\altlform$)} \textbf{or} 
%%		$\altlform\not\in\Fmc_{\fnext}$  
%%	}
%%}{return false}
%\BlankLine
%\While{$i\le s+p$}{\BlankLine
%%	Update $\Fmc_{\fnow}$ and $\Fmc_{\fnext}$, and
%%	proceed as in Algorithm~\ref{algo:ltl-sat} for input $\pa\atcq$, Lines~9 to~17\;
%		\lIf{$i>0$}{$\Fmc_{\fnow}:=\Fmc_{\fnext}$}
%		%$\Fmc_{\fnow}:=\Fmc_{\fnext}$\;
%		$\Fmc_{\fnext}:=$ Guess a set of subformulas of \altlform\;
%		
%		%\If{$i=0$ \textbf{and} \textnormal{(\textbf{\itshape not}} \textnormal{\algofont{\algoInitial}($\Fmc_{c}$, $\altlform$)} \textbf{or} 
%		%$\altlform\not\in\Fmc$\textnormal{)}}{return false}
%		
%		\BlankLine
%		\If{\textbf{not} \textnormal{{\algofont{\algoBoolCons}}($\Fmc_{\fnext}$)} \textbf{or} \textbf{not} \textnormal{{\algofont{\algoTCons}}($\Fmc_{\fnow}$, $\Fmc_{\fnext}$)}
%			%	\\$\Fmc_{p}$ is not consistent with $\Fmc_{c}$ as set of formulas subsequently satisfied according to the temporal operators
%		}{
%		return \false
%	}
%	\BlankLine
%	\If{$i=s$}{
%		$\Fmc_s:=\Fmc_{\fnow}$\;
%		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_s$}
%	\BlankLine
%	\If{$i\ge s$}{
%		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_{\Until}$ such that $\altlform_2\not\in \Fmc_{\fnow}$\;
%	}
%%	\BlankLine
%	\lIf{\colorbox{AlgoGray}{$i=n$} \textbf{and} $\pa\atcq\not\in\Fmc_{\fnow}$}{return \false}
%	\BlankLine
%	$\ax:=\Fmc_{\fnow}\cap\pv$\;\BlankLine
%	%	$\overline{\ax}:=\pv\setminus\Fmc_{c}$\;
%	\lIf{$i>n$}{$\Amc_i:=\emptyset$}\BlankLine
%	%	Initialize \textbf{additional parameters}\;
%	
%	\If{\textbf{not} \colorbox{AlgoGray} {\textnormal{\algofont{\algoTesting}($\atcq,\aont,\Amc_i,d,i,s,p,\ax$)}}}{%\colorbox{AlgoLightGray}
%		{return \false}}
%	%	$r:=$ \false if one of the \textbf{r-Satisfiability tests} fails, otherwise \true\;
%	%	\lIf{$r=$ \false}{return false}
%	\BlankLine
%	$i:=i+1$\;
%	%	Continue as in the loop of Algorithm~\ref{algo:ltl-sat}, Line~13\;
%	%	\lIf{$i=s$}{$\Fmc_s:=\Fmc_c$}
%	%	\BlankLine
%	%	\If{$i\ge s$}{
%	%		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_{\Until}\cup\Fmc_{c}$ so that $\altlform_2\not\in \Fmc_{c}$\;
%	%	}
%}
%\If{$\Fmc_{\Until}=\emptyset$ \textbf{and} \textnormal{{\algofont{\algoTCons}}($\Fmc_{\fnow}$, $\Fmc_{s}$)}
%}{
%return \true}
%return \false
%
%\caption{Procedure for Deciding TCQ Satisfiability}
%\label{algo:tq-sat}
%\end{algorithm}
%
More specifically, our contributions are as follows:
\begin{itemize}
\item 
We propose a new, general procedure for solving the TCQ satisfiability problem in polynomial space w.r.t.\ combined complexity based on adapting the algorithm originally proposed for solving the LTL satisfiability problem, which is specified in Algorithm~\ref{algo:ltl-sat}.
Recall that the latter algorithm iteratively constructs a model for a given LTL formula~\altlform: it considers a sequence of exponentially many time points~$i$, iteratively regards each of them, guesses a world~$w_i$, and describes polynomial-space tests ensuring the adequacy of $w_i$ (i.e., regarding the worlds guessed in previous steps) and relying on a polynomial amount of information that is kept and updated during the iteration.
%To construct a model for a given TQ w.r.t.\ a TKB, w
We extend that algorithm to iteratively construct a model for a given TCQ w.r.t.\ a TKB. % as it is described in Algorithm~\ref{algo:tq-sat}.
That is, Problems~\ref{def:tqa-task-obtaining} and \ref{def:tqa-task-ltl} are solved in general for $\pa\atcq$, independently of \adl; specifically, %(i)~
we use the world~$w_i$ guessed in the original algorithm%
\footnote{Recall that $w_i$ is determined by $\Fmc_\fnow$.} to determine the element~$W$ of \as that represents the CQs satisfied at ${i}$, and $\iota$.%
\footnote{To determine $\iota$ in this way, we have to ensure that the first $n$ time points are considered. This can be done by guessing the start~$s$ of the period such that it is large enough. We also have to require that $\pa\atcq\in\Fmc_{\fnow}$ when $i=n$ instead of when $i=0$.}
But our procedure still has to be tailored to the specific DL %problem 
under consideration %(e.g., TCQ entailment in \EL) 
regarding Problem~\ref{def:tqa-task-dl}. Our approach is sketched in Algorithm~\ref{algo:tq-sat}. The highlighted parts represent the critical extensions of Algorithm~\ref{algo:ltl-sat} (i.e., extensions that may influence correctness or complexity); the \colorbox{AlgoGray}{functions} which target the r-satisfiability testing are specified later in this work for each considered problem individually.

In particular, this r-satisfiability testing has to be done as follows for obtaining a concrete, polynomial-space algorithm: %\algofont{\algoPreprocessing} an d
\begin{itemize}
\item It can rely on a \emph{polynomial amount} of \emph{additional data}\index{additional data}~$d$ %---we all it an \emph{r-complete tuple}---
which is guessed in the beginning and kept during the iteration.
\item It must be done in tests that require only polynomial space and, during the iteration, may consider only one world~$W$---different from the test described in \rwlem\ref{prop:tcq-r-sat-iff}, which considers the exponential set~\as as a whole.
\end{itemize}
%the r-satisfiability testing can only rely on a polynomial amount of information, we all it an \emph{r-complete tuple}, which is guessed in the beginning and may be kept during the iteration---different from the test described in \rwlem\ref{prop:tcq-r-sat-iff}, which considers the exponential set~\as as a whole.
% out of our methodology, 
%r-satisfiability must be decidable during the iteration in tests that require only polynomial space; may consider $W$; and rely only on a polynomial amount of information, we all it an \emph{r-complete tuple}, which is guessed in the beginning and may be kept during the iteration---different from the test described in \rwlem\ref{prop:tcq-r-sat-iff}, which considers the exponential set~\as as a whole.
%Corollaries~%\ref{cor:elltl-ub-pspace}, \ref{cor:elltl-ggci-ub-pspace}, 
%\ref{cor:eltcqs-cc:wo-rigid-roles} and~\ref{cor:dlltcqs-cc} are obtained based on this new approach.
\item 
The characterizations of r-satisfiability by such a polynomial amount of information and conditions that can be tested by using only polynomial space presents another main contribution of our work. This is because we also target low complexities w.r.t.\ \emph{rigid symbols}.
%, regarding satisfiability in \EL-LTL with global GCIs (Section~\ref{sec:elltl-ggci-r-sat-charact}), and TCQ entailment in \EL (Section~\ref{sec:eltcqs-cc-rsat}) and Horn fragments of \DLLite (Section~\ref{sec:dlltcqs-r-sat-charact}). 
The common idea of our characterizations is to adapt %the conditions from 
Definition~\ref{def:tqa-r-sat}: we look for similar interpretations but consider their domains to be disjoint w.r.t.\ the unnamed individuals; and we use the additional data and test conditions to achieve the effects of the shared domain (\domfuncs\ref{eq:tqa-domfunctinds} and~\ref{eq:tqa-domfunctchis}). 
%\todo{krom dc?}
\item 
For obtaining tractable data complexity regarding TCQ entailment in \EL and Horn fragments of \DLLite, we also integrate the tests described in \rwlem\ref{prop:tcq-sat-iff} into the construction of \as and $\iota$.
The main achievement represents the algorithm we propose for \DLLite; there, we include rigid symbols and target the sublinear \ALogTime complexity.
%These results are stated in Theorems~\ref{thm:eltcqs-dc:ub:wo-rigid} and \ref{thm:dlltcqs-dc-alotime}.
\item 
The remaining containment results are rather straightforward consequences of \rwlem\ref{prop:tcq-sat-iff} and the above observation that, if rigid symbols are disregarded, the r-satsifiability test can be split into exponentially many satsifiability tests, each regarding only polynomially large conjunction of CQ literals. %  ~\ref{prop:tqa-tq-sat-containment} (some): 
%Corollaries~\ref{cor:dlltl-rigid}, \ref{cor:eltcqs-cc:ub:w-rigid-roles}, and \ref{cor:eltcqs-dc:ub:w-rigid-names}, and Theorems~%in all before only sizes interest...
%\ref{thm:dlltcqs-krombool-cc:ub-w/o-rigid} and~\ref{thm:dlltcqs-krombool-cc:ub-rigid-concepts}. %r sat bit more complex
\item 
Another major contribution are the various hardness results, where we apply the few means these lightweight DLs offer for showing hardness for \coNP, \NExpTime, \coNExpTime, and \TwoExpTime in the presence of rigid symbols.
%Theorems~\ref{thm:elltl-lb-rc}, \ref{thm:eltcqs-cc:lb:w-rigid-roles}, \ref{thm:eltcqs-dc:lb:w-rigid-names}, \ref{thm:dlltcqs-krom-cc:lb-rigid-concepts}, and
%\ref{thm:krom-cc:lb-rigid-roles}.
\item For TCQ entailment in \DLLite logics between \DLLitekrom and \DLLitehbool, we establish close relationships to TCQ entailment in more expressive DLs. %Lemmas~\ref{lem:krom-transf} and~\ref{lem:from-dl-lite-to-shq}.
\end{itemize}

%Note that the following chapters refer to the preliminaries but are self-contained otherwise. This is why explanations in different chapters may overlap due to the above described similarity of the approaches.

Below, we list the assumptions we make throughout the article are---recall that all of them are without loss of generality:
\begin{itemize}
\item Individual names are always rigid.
\item Concept and role names occurring in an ABox of a (T)KB also occur in its ontology.
\item Individual names occurring in a TCQ also occur in the ABoxes of the (T)KB regarded.
%\todo{do we have to require them to be contained in every single ABox of a TKB... because of the rewriting?}
\item CQs are connected.
\item CQs contained in a TCQ are Boolean and do not share variables; this also applies to multiple occurrences of one CQ.
\end{itemize}
%
Especially note that, if we refer to settings without rigid symbols or with only rigid concept names, this does not include the individual names.

%\todo{is the below ok? is that a linear reduction?}	
Lastly, observe that a rigid concept name $A$ can easily be represented using a flexible concept name $A'$ and a rigid role name $R_A$: by replacing every occurrence of $A$ by $A'$ and by adding the CIs $A'\sqsubseteq \exists R_A.\top$ and $ \exists R_A.\top\sqsubseteq A'$ to the ontology. This means that TCQ satisfiability in the presence of rigid concept names can be linearly reduced to TCQ satisfiability in the presence of rigid role names; specifically, 
%; that is, they are %. That is, %in \adl-LTL, the latter are %prefixed by $\Boxf$ and added as conjuncts to the formula and, regarding TCQs, they are 
%added to the ontology.
%%In the context of Chapters~\ref{ch:elltl} to~\ref{ch:exdlltcqs}, where all the considered 
%Since all DLs we consider allow to express such CIs and we generally %and global CIs can be expressed in both settings we investigate, DL-LTL satisfiability and TCQ entailment w.r.t.\ 
%regard a TKB (with non-empty ontology), we can state the following fact.
%\begin{fact}\label{fact:tqa-nrcnrr}
%	TCQ satisfiability in the presence of rigid concept names can be linearly reduced to TCQ satisfiability in the presence of rigid role names.
%\end{fact}
%
hardness results for the case $\NRC\neq\emptyset$ also apply to the case where $\NRR\neq\emptyset$. We therefore disregard the case where $\NRC=\emptyset$ but $\NRR\neq\emptyset$. %Note that we in the following proceed in this way, without explicitly referring to Fact~\ref{fact:tqa-nrcnrr}.

%\subsection{Related Work}
%\label{sec:tqa-related-work}
%
%In this section, we review related work on temporal ontology-based data access that is closest to our work, where the ontologies are written in DLs. %Note that there is no common definition of the notion temporal DL, which is why we use it in a general way for approaches explicitly integrating temporal aspects into DLs. 
%In general, there are various ways to represent time in DL modeling; for example, by considering time points as concrete datatypes~\cite{BaH-IJCAI91:cds,Lutz-IJCAI01:concdomintervals} or formalisms inspired
%by action logics~\cite{AF-JAIR98:actions,HCMGMF-JAIR13:actions}. Good overviews of different such approaches are provided in~\cite{AF-AMAI00:survey,AF-Handbook05}. 
%%The Description Logic Handbook also provides a summary  
%%More recent studies in such directions \dots
%%\todo{ask benjamin. stefan?}
%%\todo{(for me) specify survey content,also refer to dl handbook, many dim modal book}
%
%%There is no common definition of the notion \emph{temporal description logic}, which is why we use it in a general way for approaches explicitly integrating temporal aspects into DLs.
%
%We focus on \emph{temporal description logics}\index{description logic!temporal} that are combinations of standard temporal logics with DLs and focus on two-dimensional semantics, which is nowadays the general approach and common understanding of the notion (see Definition~\ref{def:tqa-tint} and the part below); though, there is no formal definition.%
%\footnote{Note that temporal description logics represent special kinds of extensions of DLs with modal logics~\cite{GKWZ03:manydimmodal}.} % (see also~\cite{dlhandbook07} for a description of the relationship).}
%Such combinations still offer a wealth of degrees of freedom:
%\begin{itemize}
%	\item base DL;
%%	\item Notion of time (e.g., based on points or intervals)
%	\item temporal logic (e.g., LTL or CTL, which is shortly covered later in this section); %, CTL%
%%	\footnote{CTL is a branching-time temporal logic that extends LTL in that }, etc.).
%	\item application of temporal logic operators: for temporalizing concepts or roles (i.e., if the operators are allowed within concept or role expressions); axioms, such as in \adl-LTL; or queries, such as in TQs;
%	%	{\hfill\myex{$\excten \sqsubseteq \Diamond_{\textit{F}}\exists\exrthr.\excele,$}\\\vspace{-0.35cm}
%	%		\hfill\myex{$\Next(\excten\sqsubseteq\exists\exrthr.\excele)$}}%
%	%	\vspace{-0.35cm}
%%	\item Additional constraints (e.g., rigid symbols).
%	\item semantics (e.g., standard first-order semantics or \emph{epistemic semantics}\index{epistemic semantics}, which separate the temporal and DL dimension (see \cite{CGLLR07:epistemic}, for example)).
%	%\onslide<5->{(e.g.\ rigid roles)\hfill%
%	%	{$\rightarrow$ rigid roles (rr)\hfill%
%	%		\myex{$\exrfou(\exifiv,\exisix)$}}%
%	%	%TODO domain?
%	%	\vspace{-0.35cm}
%\end{itemize}
%Note that the choice of temporal logic fixes the notion of time considered (e.g., if it is based on points or intervals) and that the semantics also specifies details such as if the notion of time is based on the naturals, integers, or reals; and bounded to the past or future. However, we do not further consider specifics such as the latter since their relevance is minor w.r.t.\ the results we review.
%%All point-based approaches we regard consider the natural numbers and, if not otherwise stated, bounded past and infinite future.
%%\todo{
%%	how to integrate:
%%	The temporal interpretations defined above assume discrete
%%	linear time that is bounded to the past and unbounded
%%	to the future. Of course, there are many other models of
%%	time: to obtain Dedekind-complete time, one can replace
%%	
%%	with the real numbers; to give up infinite future, one can
%%	use finite (but unbounded) initial parts of
%%	, etc. To keep
%%	things simple, however, we mainly use (N, <) as our model
%%	of time and only deviate from it when necessary
%%	}
%Moreover, the approaches in the literature differ w.r.t.\ the problem and kind of complexity they focus on.
%
%Earlier works investigate temporal versions of standard reasoning problems w.r.t.\ combined complexity and target applications such as terminologies with temporal aspects or temporal conceptual modeling. In contrast, most recent investigations focus on query answering with the goal of retrieving (temporal) data and also consider data complexity. In the following, we cover both directions. 
%
%Regarding the problems studied, we apply the terminology of the atemporal setting (e.g., the satisfiability problem of a concept w.r.t.\ a TKB is defined in correspondence with Definition~\ref{def:prelims-problems-standard}). Moreover, we also consider TKBs where the concepts and roles in the ontology are temporalized, thus extending the TKBs from Definition~\ref{def:tkb-syntax}.
%To avoid confusion, we may further slightly adapt the original names of the logics since there is no common naming scheme. Generally, we prefix DLs with the letter T if the logic allows for temporalizing concepts---we mention the temporal logic used---and add a corresponding superscript if only a subset of the temporal logic operators is allowed; the suffix -LTL denotes the fact that axioms may be temporalized with LTL operators.
%
%%for practivcal see intro, temp db logics ig?? ASK toman? 
%%abstract temp db
%%Other relevant applications
%%of DLs include the representation of and reasoning
%%about conceptual database models. Notably, extended
%%entity-relation (EER) models and UML class diagrams can
%%be embedded into DLs, and DL reasoners can be used to
%%verify their consistency and to derive implicit consequences
%%of the model [16].
%%In many applications of DLs, temporal aspects play an
%%important role. For example, the description of a concept in
%%an ontology often involves reference to temporal patterns—
%%consider, e.g., the definition of Malaria in a bio-medical
%%ontology. Likewise, time plays a crucial role when using
%%DLs to represent conceptual models of temporal databases.
%%These observations have resulted in a rather diverse literature
%%on temporal description logic (TDLs). Proposals
%
%%atsql toman allg?
%%abstract temp db
%%datalog, rules?
%%abgrenzen von temp logik, keine fact base , rigid symbols. elltl? 
%%temp dbs
%
%%\todo{should I mention sth like: With formalisms that are similar to the ones we consider, we sometimes give hints on how the results have been obtained to point out the differences with our proceeding}
%
%%recently focus shifted to lightweight and non-standard
%%can coarsely discern though overlabs weg combis
%\subsubsection{Reasoning with Temporalized Concepts and Axioms}
%
%The first combination of a DL and a point-based temporal logic, based on a two-dimensional semantics, has been proposed in~\cite{Schild93}.
%Subsequent studies then have focused on classifying different combinations of LTL and (extensions of) \ALC regarding expressivity and complexity, with results mostly in the range of \ExpSpace, if rigid roles are disregarded. Since a detailed discussion of these results is beyond the scope of this work, we refer to \cite{GKWZ03:manydimmodal,AF-Handbook05} for details;
%the Description Logic Handbook~\cite{dlhandbook07} also provides a summary of main results.
%%%The 
%%Early works investigate several combinations of standard temporal logics with extensions of \ALC regarding standard reasoning problems with results mostly in the range of \ExpSpace; for details, we refer to \cite{rwlemma}. 
%An important outcome of that research is however the observation that rigid roles or several other constraints on roles (e.g., temporal operators) generally lead to undecidability.
%%
%Because decidability represents one major feature of DLs, research since then has been dedicated to the study of decidable temporal DLs, which we review in the following. Decidable temporal DLs are generally obtained by either restricting the expressivity of the temporal features (e.g., restricting the operators or rigid symbols allowed) or the DL (e.g., by focusing on lightweight DLs). %Yet, m
%Most recent studies often consider restrictions on both sides since they target tractable logics. %, to lightweight formalisms.
%
%%\todo{$LTL_{\ALC}$}
%\cite{LuWZ-TIME08:survey} show that, without rigid symbols, neither temporalizing \ALC concepts nor GCIs leads to an increase in complexity over the \ExpTime complexity of satisfiability in \ALC. Note however that rigid concept names~$A$ with the former kind of temporalization can be modeled with GCIs of the form $A\sqsubseteq \Boxf A$.
%While the temporal and description logic part thus cannot interact critically in these formalisms, the combination of the two allows intricate interactions and leads to \ExpSpace-completeness. In a nutshell, this is the case because the LTL part, which generally leads to a model (i.e., a DL-LTL structure) that is periodic with a period of exponential length, here does not have this property any more; formulas as the following example from~\cite[p.~8]{LuWZ-TIME08:survey} have only models whose interpretations all must be distinct: %Sec 4.2
% $$\Boxf(\lnot(\top\sqsubseteq\lnot A)\land(A\sqsubseteq\Next\Boxf\lnot A)).$$
%
%%focus on different temporal versions of \ALC based on LTL and show that,
%
%Temporalized DL axioms (see Section~\ref{sec:tqa-elltl}) have originally also been proposed regarding \ALC \cite{BaGL-TOCL12}. The satisfiability problem in \ALC-LTL similarly has the same complexity as in the atemporal case, but rigid concepts and roles lead to \NExpTime and \TwoExpTime-completeness, respectively, and thus to a considerable increase in complexity. 
%In the same paper, it is however also shown that this increase can be overcome, at least for rigid concepts, if GCIs are only allowed to occur globally in the formulas. %that is, the formulas must be conjunctions in which GCIs may only occur as conjuncts prefixed by the $\Boxf$ operator. This logic is %called \ALC-LTL with global GCIs and 
%%denoted by \ALC\ggci-LTL.
%%
%\cite{phdmarcel} extend the former results to \SHOQ-LTL, which implies that they hold for all such temporal DLs based on a DL between \ALC and \SHOQ.
%
%Tractable DLs in combination with LTL are investigated in \cite{AKLWZ-TIME07:temporalising,AKRZ-TOCL14:cookbook}.
%\cite{AKRZ-TOCL14:cookbook} investigate the KB consistency problem for several temporal extensions of different \DLLite logics %
%%\footnote{
%%	The problem is defined as in Definition~\ref{def:prelims-problems-standard} but w.r.t.\ temporalized concepts, also in the KB.
%%}
%that allow for temporalizing concepts with subsets of LTL operators, including rigid roles.
%%
%%goal app recently 
%%temporal conceptual data models (TCMs) depending on the available
%%modelling constructs. O
%The positive results include containment in \NLogSpace or \PTime and are obtained by reduction to %clausal 
%fragments of propositional temporal logic, but they only hold for formalisms strongly constrained on the temporal side. In most cases, more variety in that direction leads to \NP-completeness and, if more expressive role expressions are allowed (e.g., arbitrary RIs), even to undecidability.
%%, which opens a way to employ propositional or
%%first-order temporal provers for reasoning about temporal data models
%%
%Regarding both \DLLite and \EL, 
%\cite{AKLWZ-TIME07:temporalising} integrate temporalized concepts, axioms, and rigid roles. 
%They show that the satisfiability of formulas in this setting for the resulting logics $\textit{TDL-Lite}_\textit{bool}$-LTL and $\textit{TDL-Lite}^{\Next}_\textit{horn}$-LTL is \ExpSpace-complete, whereas it is \PSpace-complete in $\textit{TDL-Lite}^{\Next}_\textit{krom}$-LTL; $\textit{TDL-Lite}_\textit{bool}$ denotes the temporal extension of \DLLitebool where the concepts in CIs may be formed by applying full LTL to basic concepts while, in the latter two formalisms, only \Next may be applied. % to the concepts.
%The logics thus allow to describe necessary future consequences in the ontology; for example, the fact that, an application that is out of user focus during two consecutive observations, should be in the energy saver mode at the next observation moment, can be expressed as follows:
%%in a room that has no occupants during two consecutive observations, the lights should be switched off at the next observation moment, can be expressed as follows:
%%$$\xcRoom\sqcap\lnot\xrHasoccupant.\top\sqcap\Next\lnot\xrHasoccupant.\top\sqsubseteq
%%\Next\Next\xcLightsoff.$$ 
%$$\xcApp\sqcap\xcOutoffoc\sqcap\Next\xcOutoffoc\sqsubseteq
%\Next\Next\xcESM.$$ 
%%\todo{the negation can be modelled in \DLLite, right?\\what example do you like better?\\for me: above hasstate}
%Note that, in all these formalisms, rigid concept names~$A$ can be modeled by adding conjuncts of the form $\Boxf(A\sqsubseteq \Next A)$ to the formula.
%%They show that the satisfiability problem in this setting for both LTL$_{\DLLitebool}$-LTL and LTL$^{\Next}_{\DLLitehorn}$-LTL is \ExpSpace-complete, whereas it is \PSpace-complete in $\atl_{\DLLitekrom}$-LTL.%
%%\footnote{Note that in LTL$^{\Next}_{\DLLitehorn}$ and LTL$^{\Next}_{\DLLitekrom}$ not full LTL but only the \Next operator may occur within the (then temporalized) CIs.}
%%
%The results of \cite{AKLWZ-TIME07:temporalising} are interesting because, in the atemporal case, complexity results for \DLLitekrom are usually worse than corresponding ones for \DLLitehorn \cite{dllrelations}.
%In a nutshell, $\textit{TDL-Lite}^{\Next}_\textit{horn}$ CIs are critical because they allow to encode a standard counter---over time---that discerns exponentially many time points per individual (e.g., similar to the counter in the proof of Theorem~\ref{thm:krom-cc:lb-rigid-roles}); in addition, the outer LTL allows to specify conditions that hold for all individuals \emph{per time point}; and additional restrictions on selected individuals, which are based on former time points, may constrain the latter conditions further. 
%Note that this interaction does not depend on rigid roles.
%The other results are again based on translations into fragments of first-order temporal logic. 
%%\todo{is the explanation too detailed or incorrect?}
%%
%For $\Tmc{\EL}^{\Diamondf}$, a logic allowing for temporalized concepts that are standard \EL concepts augmented with the operator $\Diamondf$, subsumption is shown to be undecidable in the presence of rigid roles; the point is that $\Diamondf$ in concept expressions in combination with the \EL features allows to model disjunction and hence to reduce to an undecidable temporal version of \ALC.
%%
%For that reason, the complexity of the \EL-LTL satisfiability problem was an interesting open question since the logic represents another temporalization of the popular DL \EL and there was no hardness result apart from the \PSpace complexity of LTL. 
%%
%We address \EL-LTL %complete the complexity picture for temporalized DL axioms for these tractable DLs 
%in~\cite{BoT-IJCAI15}, where we investigate complexity w.r.t.\ different selections of rigid symbols and
%show that \EL-LTL can be allocated in between \DLLite-LTL and \ALC-LTL/\SHOQ-LTL.
% % by investigating \EL-LTL and \EL\ggci-LTL.
%These results together with new ones on \DLLite-LTL and other such temporal lightweight DLs are detailed in Chapter~\ref{ch:elltl}.
%
%There are some recent works that temporalize concepts with temporal logic operators different from the LTL ones. \cite{GuJuL-ECAI12:ctl,GuJuS-KR14:marriage,GuJuS-IJCAI15:tdls-tboxes} consider \emph{computation tree logic} (CTL)~\cite{ClarkeE81:ctl} for temporalizing concepts and investigate subsumption.
%CTL extends LTL in that the time is not considered to be linear regarding future, but branching. Since it allows to quantify over these branches both existentially and universally, it allows to model alternative future behavior. For example, the fact that a dishwasher that is currently filled by someone may be switched on in the next observation moment can be expressed with the following CI: $$\xcDishwasher\sqcap\exists\xrIsfilled.\top\sqsubseteq\mathbf{E}\Next \xcSwitchedon$$
%where $\mathbf{E}$ denotes the existential path quantifier.
%The latter expresses that the statement following it %(i.e., $\Next \xcSwitchedon$) 
%represents a possible future, while other future states may exist though.
%%
%\cite{GuJuL-ECAI12:ctl} show that, if CTL is applied to \ALC, then the complexity does not increase over the atemporal case %; regard a combination with temporalized axioms; 
%and propose a tractable temporal DL based on \EL, %that admits polynomial-time reasoning, but is 
%which is however very restricted.
%Moreover, the results are very negative---nonelementary or undecidable---if rigid roles are allowed, even for \EL \cite{GuJuS-KR14:marriage}. For that reason, follow-up investigations~\cite{GuJuS-IJCAI15:tdls-tboxes} consider restricted ontologies (e.g., acyclic ones) and, indeed, obtain better results. Nevertheless, containment in \PSpace, for instance, is only achieved by either strongly restricting the allowed temporal operators or disregarding the ontology entirely.
%
%A new direction of research has recently been pursued in \cite{GuJO-ECAI16:metric}, investigating \emph{metric} versions of LTL for temporalizing \ALC concepts (and GCIs) and regarding satisfiability (of the resulting ontological formulas). One such logic allows, for example, to annotate $\Until$ with an interval based on concrete values, representing time points.
%% that restricts the % %truth in an 
%%interpretation to the corresponding time points. 
%Yet, the complexities are rather high, often in the range of \ExpSpace and \TwoExpSpace.
% %http://www.informatik.uni-bremen.de/~jeanjung/pub/GJO16.pdf
%While the paper presents important foundational work on metric temporal DLs, the authors themselves state that the need for similar studies regarding lightweight DLs, query answering, and data complexity to analyze the applicability for practical temporal OBDA.
%
%Observe that the above described results also apply to instance query answering (i.e., the problem of instance checking), as it is the case in the atemporal setting.  The works do however not investigate data complexity, which is relevant in practice. The next described more recent studies address this issue. 
%
%\subsubsection{Querying for Temporal Data}%numerous
%\index{query answering}
%
%Query answering with the goal of retrieving data % (tuples of) instances 
%is in focus of recent research in DLs, in general, and this is reflected in the latest explorations on reasoning about temporal knowledge. The different works are primarily discerned regarding the ontology considered, depending on whether it is also temporal %~\cite{AKKRWZ-IJCAI15:omtqs,GuJK-ICAI16-tel} 
%or written in a classical DL. %~\cite{BaBL-JWS15,BaBL-AI16,BoLT-JWS15,BoT-IJCAI15,BoT-GCAI15}. 
%The former approaches offer more expressivity but, on the other hand, tend to lead to higher reasoning complexities. For this reason, they are usually studied w.r.t.\ lightweight DLs.
%%\todo{reicht es wenn ich da ein paar nenne, und unten mehr diskutiere?}
%
%%Note that the problem in focus is usually temporal query answering entailment
%
%%CAN MODEL RIGID ROLES IN THEIR RIS!
%% results are obtained by 1 translating NFAs to rewritings, also using 2 (temporal) canonical models 3 constructing rewritings based on the latter (oder so in der art) 
%\cite{AKKRWZ-IJCAI15:omtqs} investigate different temporal extensions of the \DLLite logics described in Section~\ref{sec:prelims-dls}.% regarding first-order rewritability of the temporal query answering problem.%
%\footnote{Note that \cite{AKKRWZ-IJCAI15:omtqs} actually study fragments that are slightly more expressive than those described in Section~\ref{sec:prelims-dls} (e.g., they consider more expressive RIs that may even model rigid roles). }
%The goal of the work are first-order rewritability results regarding the temporal query answering problem (see Definition~\ref{def:prelims-fo-rew}). The queries are arbitrary combinations of temporalized concept and role atoms using the operators of first-order temporal logic and thus very expressive, which is why epistemic semantics are employed (i.e., it is well known that queries with negation are not tractable, even in the atemporal setting~\cite{GIKK-JWS15}). 
%%
%However, the investigations then mainly consider a very restricted setting where roles are disregarded and the ABoxes contain a single individual name only (the name itself may occur multiple times in an ABox). Though, these results can, amongst others, be applied to show first-order rewritability of instance query answering in $\textit{TDL-Lite}^{\Next}_\textit{core}$ and $\textit{TDL-Lite}^{\Boxf}_\textit{core}$. In particular, \cite{AKKRWZ-IJCAI15:omtqs} define specific temporal canonical interpretations for TKBs in these logics, which can be used to construct the rewritings.
%%Note that, while the above described results have mainly been shown by translating to fragments of first-order temporal logic, the constructions in \cite{AKKRWZ-IJCAI15:omtqs}, amongst others, construct rewritings based on specific temporal canonical interpretations, which exist for the latter two logics. %translate NFAs into rewritings to model the temporal behavior (of elements) specified in the ontology and use temporal canonical interpretations
%% and to get abstract transfer results (i.e., results that identify conditions under which first-order rewritability of the queries is preserved for combinations of LTL with DL-Lite. ).
%%most results presented in the work only apply to a very restricted setting where roles are disregarded and the ABoxes contain a single individual name only.
%%\todo{can I drop the abstract transfer results (not mentioned currently)?}
%%\todo{maybe an example formula, which is not possible with TCQs}
%
%Also for TKBs where the ontology is written in $\mathcal{TEL}^{\Nextstar}$ (i.e., the logic allows for both \Next and \Previous), there are canonical models, which can be used to show that the satisfiability problem is tractable w.r.t.\ data complexity if rigid roles are disallowed \cite{GuJuK-IJCAI16:tel}. The latter paper also identifies a certain \emph{periodicity} of the ontology to ensure decidability and proposes several acyclicity notions for ontologies in temporal \EL that yield tractable combined and data complexity.
%%shows that the data complexity is in \PSpace---including rigid roles---if the ontology is particularly \emph{periodic}.  and proposes acyclicity conditions.
%%FO rewritable if tbox acyclis
%%
%%proposes  consider instance query entailment in different temporal extensions of \EL with the goal of identifying fragments where data complexity is tractable. 
%%They also refine the results of \cite{} by showing that TEL.. is undecidable even w.r.t.\ data complexity. 
%%\todo{do we have to detail that?}
%
%Research in the second direction---temporal query answering regarding classical onto\-logies---has been first considered in a general way in~\cite{GuKla-RR12:approach} regarding expressive operators on both the temporal and the DL side (i.e., first-order formulas). 
%%
%{Temporal conjunctive queries} have first been studied in \cite{BaBL-CADE13}, focusing on the complexity of the entailment problem. That paper and follow-up investigations~\cite{BaBL-JWS15,BaBL-AI15} focus on \ALC and extensions such as \SHOQ---under open world semantics---, which is reflected in the rather high complexity results. Yet, for many of the considered DLs the data complexity is in \coNP, as in the atemporal case, even in the presence of rigid concept names. Observe that the exact complexity w.r.t.\ rigid roles is still open, but containment in \ExpTime is known. The combined complexity is generally as in the atemporal case if rigid symbols are not considered, but w.r.t.\ rigid symbols increases up to \TwoExpTime. 
%
%Together with \cite{Klarman-LPAR13:sql,KlaM-RR14:sql} we regard TCQ answering and entailment w.r.t.\ the most prominent lightweight description logics~\cite{BoLT-JWS15,BoT-IJCAI15,BoT-GCAI15}. 
%%
%Our complexity results on TCQ entailment~\cite{BoT-IJCAI15,BoT-GCAI15} are detailed in Chapters~\ref{ch:eltcqs}, \ref{ch:dlltcqs}, and~\ref{ch:exdlltcqs} regarding \EL, \DLLitecore to \DLLitehhorn, and extensions of \DLLitehhorn, respectively; note that especially w.r.t.\ combined complexity, the latter logics have however turned out to be not very ``lightweight'' any more.  In Chapter~\ref{ch:tqs}, we describe the initial parts of the work in~\cite{BoLT-JWS15}, by generalizing TCQs and proposing a practical approach for temporal query answering; for details about algorithms, especially including rigid concept names, we refer to the paper. In a nutshell, the feasibility of rewriting is achieved by dropping the negation operator.
%%
%\cite{Klarman-LPAR13:sql,KlaM-RR14:sql} also describe an approach for implementation w.r.t.\ \DLLitecore, but achieve the first-order rewritability by considering epistemic semantics.
%Note that there are also some works on non-standard reasoning problems regarding TCQs that are different from query answering and entailment~\cite{KlaM-LPAR13:streams,KlaM-DL14:abduction}. There, the focus is on ABox {abduction}, which roughly is the question of how the given ABox sequence can be extended so that a specific TCQ is entailed.
%%\todo{Do I have to mention that KlaM-LPAR13:streams use sort of temporalized concepts in their temporal rules?}
%
%Observe that, although the above described queries considered in \cite{AKKRWZ-IJCAI15:omtqs} are very expressive, they do not subsume TCQs. TCQs allow to existentially quantify variables occurring in conjunctions of atoms, whereas the other queries can only express tree-shaped CQs, via concept expressions.
%
%A similar observation can be made regarding the logics where the axioms are temporalized. While formulas containing only temporalized assertions %(e.g., $Application(a)\land \Next \dots$) 
%can be directly regarded as TCQs, the latter cannot express local CIs. On the other hand, CQs that are not tree-shaped (e.g., see the introductory example CQ~\eqref{eq:intro-cq}) cannot be modeled through concepts in logics such as \ALC-LTL.
%
%There are also some recent proposals of interval temporal description logics that allow for tractable query answering \cite{ABMSR-ECAI14:tdll-interval,%dllbool... expspace
%	AKRZ-AAAI15:interval}. %hhorn %,KPPRZ-IJCAI16-interval}. 
%Specifically, they combine fragments of the Halpern-Shoham interval logic~\cite{HalpernS91:interval-logic} with \DLLite. 
%%second paper:While the proposed formalisms are rather restricted (e.g., $\exists R$ on the right-hand side of CIs is disallowed)
%Note that this setting is rather different from the one we consider. Nevertheless, these approaches follow an interesting direction of research, given that, for example, 
%the possibility to associate data with intervals has been recently incorporated into the SQL standard~\cite{KM-SIGMODR12:temporal-sql}.
%% and Datalog.
%%\todo{should I mention the one work on Datalog?:http://www.dcs.bbk.ac.uk/~roman/papers/HS-IJCAI16.pdf}
%%% tractable Horn fragment of the Halpern-Shoham
%%% temporal logic and extend it to interval-based temporal description
%%% logics, instance checking in which is P-complete for
%%% both combined and data complexity.
%%\todo{complete
%%	%http://www.dcs.bbk.ac.uk/~roman/papers/aaai-15.pdf %http://www.dcs.bbk.ac.uk/~roman/papers/HS-IJCAI16.pdf
%%}
%%%http://eprints.bbk.ac.uk/10332/1/IJCAI13-112.pdf
%
%%\todo{datalog1, others in that direction?}
%%\subsubsection{Temporal Description Logics}
%%
%%
%%	\begin{itemize}
%%		%		\item First proposed in 1993?!
%%		\item Diverse approaches for temporal DLs\\ %\\
%%		{$\rightarrow$ \alert{Combinations of standard logics}, two-dimensional semantics} %, const.\ domain)}
%%		\item<6-> Different reasoning problems studied $\rightarrow$ combined and data complexity
%%	\end{itemize}
%%	\medskip
%%	{
%%		\textbf{The History \dots}
%%		\begin{itemize}
%%			\item Early works focus on extensions of \ALC \cite{Gabbay03,AF-Handbook05}
%%			\item<8-> W.r.t.\ {global} ontology:\\
%%			\alert<8>{\ALC} + $\Diamond_{\textit{F}}$ \alert<8>{+ rigid roles}: Satisfiability \alert<8>{is undecidable} \cite{Gabbay03}
%%			\item<9-> %But we want to have rigid roles $\rightarrow$ 
%%			Two ways: \alert{Restrict DL or (application of) TL}
%%		\end{itemize}
%%	}
%%
%%
%%
%%%\begin{frame}[t]
%%%	\frametitle*{{\insertsection}}%\setlength{\leftmargini}{0.55\leftmargini}
%%%	\framesubtitle{Temporalized \dots}
%%	%Temporalized \dots\\
%%	{\color<6->{gray}
%%		\textbf{\dots Concepts:}} 
%%	\begin{itemize}\color<6->{gray}
%%		\item<2-> \EL + $\Diamond_{\textit{F}}$ + rr: 
%%		Subsumption is undecidable 
%%		\cite{AKL+-TIME07} %TODO  (w.r.t.\ GCIs)
%%		\item<3-> \ALC + CTL + rr: 
%%		Satisfiability is decidable
%%		if ontology restricted~\cite{%GuJS-KR14,
%%			GuJS-IJCAI15}%,Gabbay03LTL/
%%		\item<4-> \color<6->{fg}
%%		\textit{DL-Lite}$_{\textit{horn/krom}}$ + $\Next$ + \alert<8->{rr}: 
%%		Satisfiability (w.r.t.\ temporalized axioms)  %\phantom{\textit{DL-Lite}$_{\textit{horn/krom}}$ + $\Next$ + \alert<8->{rr}: }
%%		is \phantom{\textit{DL-Lite}$_{\textit{horn/krom}}$ + $\Next$ + \alert<8->{rr}:}
%%		\ExpSpace/\alert<8->{\PSpace-complete} 
%%		\cite{AKL+-TIME07}
%%		\item<4->
%%		${\textit{DL-Lite}^\Nmc_\alpha},\alpha\in\{ bool,krom, core\}$ + LTL-fragments + rr:
%%		\begin{itemize}\color<6->{gray}%TODO also for frags of LTL
%%			\item Satisfiability between \NLogSpace and \PSpace, but
%%			\item undecidable with %unrestricted 
%%			role inclusions or temporalized roles 
%%			\cite{ArtaleKRZ14} %TODO CHECK IF rigid enough%\\
%%			%interact with funct consts!
%%			%role incls tog with cana model all alc constructors
%%			%temp roles tog with tiling?!
%%		\end{itemize}
%%		\item<5-> ${\textit{DL-Lite}^{\Hmc+}_{\textit{core}}}$ + $\Diamond_{\textit{P}},\Diamond_{\textit{F}}$ (l.)/$\Previous, \Next$: Conjunctive 
%%		queries/ instance queries %FO($<$)
%%		\phantom{${\textit{DL-Lite}^{\Hmc+}_{\textit{core}}}$ + $\Diamond_{\textit{P}},\Diamond_{\textit{F}}$ (l.)/$\Previous, \Next$:}
%%		FO-rewritable \cite{AKWZ-IJCAI13,AKKRWZ-IJCAI15}
%%		%\item<5-> 	
%%		%\DLLitehcore + $\Previous, \Next$: %($\Boxm,\Box_{\textit{F}}$):
%%		%Instance queries %FO($<,+$)/FO($<$)
%%		%FO-rewritable \cite{AKKRWZ-IJCAI15} %TODO HORN? %{\footnotesize
%%		%\item<5-> ${\textit{DL-Lite}^{\Hmc+}_{\textit{core}}}$ + $\Diamond_{\textit{P}},\Diamond_{\textit{F}}$ (l.): Conjunctive 
%%		%queries %FO($<$)
%%		%FO-rewritable \cite{AKWZ-IJCAI13}
%%		%\item<5-> 	
%%		%\DLLitehcore + $\Previous, \Next$: %($\Boxm,\Box_{\textit{F}}$):
%%		%Instance queries %FO($<,+$)/FO($<$)
%%		%FO-rewritable \cite{AKKRWZ-IJCAI15} %TODO HORN? %{\footnotesize \cite{AKKRWZ-IJCAI15}}
%%		%		\item \DLLitehhorn + $\Hmc\Smc$: Instance query answering 
%%		%		\PTime-complete %(combined and data complexity)%, also for data complexity 
%%		%		\cite{AKRZ-AAAI15} %TODO + global at role
%%	\end{itemize}
%%	\smallskip
%%	\textbf{\dots Axioms}{\textbf{:} }% 	\textbf{ (LTL)
%%	{\alert{Positive results also for \EL?}}
%%	{\\\hspace*{0.4cm}\ALC + LTL: Complexity of sat. w/o rigid symbols as in atemporal case %
%%		%	between \ExpTime and \TwoExpTime%		 depending on rigid symbols, operators, \dots 
%%		\cite{BaGL-TOCL12}}
%%	\smallskip
%%	
%%	\textbf{\dots Queries]}{\textbf{:} }\onslide<9->{\alert{Good complexities for other
%%			lightweight DLs%full TCQs in the 
%%			%		\EL \& \DLLite family
%%			? } (this talk!)}%(full TCQs!)}}
%%	
%%		\begin{itemize}
%%			\item \ALC ext.: 
%%			%Rigid concepts do not increase data complexity of \alert<7>{entailment} %atemporal %case for 
%%			%%\phantom{\ALC}
%%			%\alert<7>{of \hfill temporal conjunctive queries~(TCQs)} (vs.\ atemporal)~\cite{BaBL-JWS15,BBL-AI15}
%%			%\begin{itemize}
%%			%	\item W/o rigid symbols, complexity as in atemporal case
%%			%	\item Rigid concepts do not increase data complexity \cite{BaBL-JWS15,BBL-AI15}
%%			\alert<7>{Entailment of temporal conjunctive queries~(TCQs)} 
%%			\begin{itemize}
%%				\item W/o rigid symbols, complexity as in atemporal case
%%				\item Rigid concepts do not increase data complexity \cite{BaBL-JWS15,BBL-AI15}
%%			\end{itemize}
%%			%Rigid concepts do not increase data complexity of entailment 
%%			%\phantom{\ALC- ext.: }of temporal conjunctive queries~(TCQs) 
%%			%Data com. of e
%%			%Entailment of temporal conjunctive queries~(TCQs) 
%%			%\phantom{\ALC- ext.: }(TCQs) 
%%			%w.r.t.\ rigid concepts as in atemporal case
%%			%\cite{BaBL-JWS15,BBL-AI15}
%%			\item \DLLitecore: 
%%			TCQs are \alert<9->{FO-rewritable} under epistemic semantics 
%%			\cite{KlaMe14}
%%		\end{itemize}














We close this section on LTL by describing the procedure for deciding LTL satisfiability the originally proposed in {\cite[\citesec4]{SiCl85:ltlpspace}} in Algorithm~\ref{algo:ltl-sat}, which we extend in Chapters~\ref{ch:elltl}, \ref{ch:eltcqs}, and \ref{ch:dlltcqs} to obtain our results. %
%\footnote{We present the algorithm adapted to our setting where satisfiability is to be decided w.r.t.\ at time point~$0$. The original algorithm checks satisfiability in general.
%	}
%%
\begin{algorithm}
	\KwIn{LTL formula \altlform}
	\KwOut{\true if \altlform is satisfiable, otherwise \false}
	\BlankLine
	$i:=0$\;
	$s:=$ Guess a number $\le2^{|\altlform|}$ and $>0$\;
	$p:=$ Guess a number $\le4^{|\altlform|}$\;
	\BlankLine
	$\Fmc_{\fnext}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
	$\Fmc_{\fs}:=\emptyset$, %\;
	$\Fmc_{\Until}:=\emptyset$\;
	%
	\BlankLine
	$\Fmc_{\fnow}:=$ Guess a subset of $\Clo(\{\altlform \})$\;
	\BlankLine
	\If{\textbf{not} \textnormal{{\algofont{\algoBoolCons}}($\Fmc_{\fnow}$) \textbf{or} 
			\textbf{\itshape not} \textnormal{{\algofont{\algoInitial}}($\Fmc_{\fnow}$%, $\altlform$
				)} \textbf{or} 
			$\altlform\not\in\Fmc_{\fnow}$  
		}
	}{return \false}
	%$\Fmc_{\fnow}:=\emptyset$, %$\Fmc_{c}:=\emptyset$, 
	%$\Fmc_{\fs}:=\emptyset$, %\;
	%$\Fmc_{\Until}:=\emptyset$\;
	%%
	%\BlankLine
	%$\Fmc_{\fnext}:=$ Guess a set of subformulas of \altlform\;
	%\BlankLine
	%\If{\textbf{not} \textnormal{\algofont{\algoBoolCons}($\Fmc_{\fnext}$) \textbf{or} 
	%		\textbf{\itshape not} \textnormal{\algofont{\algoInitial}($\Fmc_{\fnext}$, $\altlform$)} \textbf{or} 
	%		$\altlform\not\in\Fmc_{\fnext}$  
	%	}
	%}{return false}
	\BlankLine
	\While{$i\le s+p$}{\BlankLine
		\lIf{$i>0$}{$\Fmc_{\fnow}:=\Fmc_{\fnext}$}
		%$\Fmc_{\fnow}:=\Fmc_{\fnext}$\;
		$\Fmc_{\fnext}:=$ Guess a set of subformulas of \altlform\;
		
		%\If{$i=0$ \textbf{and} \textnormal{(\textbf{\itshape not}} \textnormal{\algofont{\algoInitial}($\Fmc_{c}$, $\altlform$)} \textbf{or} 
		%$\altlform\not\in\Fmc$\textnormal{)}}{return false}
		
		\BlankLine
		\If{\textbf{not} \textnormal{{\algofont{\algoBoolCons}}($\Fmc_{\fnext}$)} \textbf{or} \textbf{not} \textnormal{{\algofont{\algoTCons}}($\Fmc_{\fnow}$, $\Fmc_{\fnext}$)}
			%	\\$\Fmc_{p}$ is not consistent with $\Fmc_{c}$ as set of formulas subsequently satisfied according to the temporal operators
		}{
		return \false
	}
	\BlankLine
	\If{$i=s$}{
		$\Fmc_s:=\Fmc_{\fnow}$\;
		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_s$}
	\BlankLine
	\If{$i\ge s$}{
		$\Fmc_{\Until}:=$ All formulas of the form $\altlform_1\Until\altlform_2\in \Fmc_{\Until}$ so that $\altlform_2\not\in \Fmc_{\fnow}$\;
	}
	$i:=i+1$\;
	%\Fmc_{p}:=\Fmc_{c}$\;
}
\If{$\Fmc_{\Until}=\emptyset$ \textbf{and} \textnormal{{\algofont{\algoTCons}}($\Fmc_{\fnow}$, $\Fmc_{s}$)}
}{
return \true}
return \false

\caption{Procedure for Deciding LTL Satisfiability}
\label{algo:ltl-sat}
\end{algorithm}
%
In particular, \cite{SiCl85:ltlpspace} propose a nondeterministic algorithm which runs in an amount of space polynomially bounded by the formula~\altlform considered; we consider $|\altlform|$ to denote the number of symbols occurring in \altlform. The idea for constructing an LTL structure~\altlint satisfying \altlform is to iteratively guess subsets of $\Clo(\{\altlform \})$ that represent the subformulas satisfied in \altlint at each point in time. More precisely, 
every such set induces a unique world containing exactly the propositional variables that are true in the guessed set.
%This approach is complete since \cite[Theorem~4.7]{SiCl85:ltlpspace} also show that, if \altlform is satisfiable, then there must be a \emph{periodic} model of \altlform with a period that is exponential in the size of~\altlform.
%
In what follows, we describe that procedure, given as Algorithm~\ref{algo:ltl-sat}, in more detail. We thereby rely on the subprocedures below.
\todo{later directly present our extended version and move the following procedures to there?}
\begin{itemize}
	\item $\algofont{\algoBoolCons}$: Given a set~\Fmc of LTL~formulas, it checks the Boolean consistency of the latter by returning true iff the following hold for all $\altlform\in\Clo(\Fmc)$:
	\begin{itemize}
		\item $\altlform=\altlform_1\land\altlform_2\in\Fmc$ iff $\altlform_1,\altlform_2\in\Fmc$,
		\item $\altlform=\lnot\altlform_1\in\Fmc$ iff $\altlform_1\not\in\Fmc$.
	\end{itemize}
	
	\item $\algofont{\algoInitial}$: Given a set~\Fmc of LTL~formulas, % and an LTL formula~\altlform, 
	it checks if \Fmc can describe the formulas satisfied at time point~$0$ in an LTL structure by returning true iff the following hold for all $\altlform\in\Clo(\Fmc)$:
	\begin{itemize}
		\item $\altlform=\altlform_1\Since\altlform_2\in\Fmc$ iff $\altlform_2\in\Fmc$
		\item $\altlform=\Previous\altlform_1\not\in\Fmc$.
	\end{itemize}
	\item $\algofont{\algoTCons}$: Given two sets~$\Fmc_{\fnow}$ and $\Fmc_{\fnext}$ of LTL~formulas, it checks if they can be satisfied in an LTL structure at consecutive time points by returning true iff the following hold for all $\altlform\in\Clo(\Fmc)$:
	\begin{itemize}
		\item $\altlform=\Next\altlform_1\in\Fmc_{\fnow}$ iff $\altlform_1\in\Fmc_{\fnext}$,
		\item $\altlform=\Previous\altlform_1\in\Fmc_{\fnext}$ iff $\altlform_1\in\Fmc_{\fnow}$,
		\item $\altlform=\altlform_1\Until\altlform_2\in\Fmc_{\fnow}$ iff $\altlform_2\in\Fmc_{\fnow}$ or ($\altlform_1\in\Fmc_{\fnow}$ and $\altlform_1\Until\altlform_2\in\Fmc_{\fnext}$),
		\item $\altlform=\altlform_1\Since\altlform_2\in\Fmc_{\fnext}$ iff $\altlform_2\in\Fmc_{\fnext}$ or ($\altlform_1\in\Fmc_{\fnext}$ and $\altlform_1\Since\altlform_2\in\Fmc_{\fnow}$).
	\end{itemize}
\end{itemize}

The procedure is based on the fact that, if \altlform is satisfiable, then there must be a \emph{periodic} model %\index{model!periodic} 
of \altlform with a period that starts at a time point exponential in the size of~\altlform and is of length exponential in the size of~\altlform \cite[Theorem~4.7]{SiCl85:ltlpspace}. This means that the algorithm can iterate over all time points until the end of the period using a counter~$i$ that can be represented in polynomial space.
The start~$s$ and length~$p$ of the period are guessed in the beginning.%
\footnote{For simplicity, we additionally require $s>0$ in Algorithm~\ref{algo:ltl-sat}; this is clearly without loss of generality.}%, given that we consider a period.}
%
This approach works specifically %is in particular complete 
because the algorithm does not store all the sets of subformulas guessed during the iteration. Instead, it focuses on only four such sets $\Fmc_{\fnow}$, $\Fmc_{\fnext}$, $\Fmc_{\fs}$, and $\Fmc_{\Until}$, which are updated during processing and occupy only a polynomial amount of memory. $\Fmc_{\fnow}$ specifies~\altlint w.r.t.\ the present time point $i$, $\Fmc_{\fnext}$ describes the world for the next time point, $\Fmc_{s}$ the one for time point $s$, and $\Fmc_{\Until}$ is used as auxiliary set.
%
$\Fmc_{\fnow}$ is guessed in the beginning and it is checked if this set can describe the formulas satisfied at time point~$0$ in an LTL structure that is a model of \altlform. 
%
Subsequently, the counter is continuously incremented and, until it reaches the beginning of the period~$s$, in each
step: $\Fmc_{\fnow}$ and $\Fmc_{\fnext}$ are updated, which means that a set of subformulas of~\altlform is guessed for the latter; further,
%
the Boolean consistency of the new set, and its consistency with the set
for the present time point (according to the temporal operators) are checked.
Regarding the latter, note that the satisfiability test for subformulas of the form $\altlform_1\Until \altlform_2$ may be deferred to the next iteration step if $\altlform_1\in\Fmc_{\fnow}$.
%(e.g., if $\altlform_1\Until \altlform_2\in\Fmc_{p}$, then we must either have $\altlform_2\in\Fmc_{p}$ or $\altlform_1\Until \altlform_2\in\Fmc_{c}$, so that the satisfiability test of the $\Until$-formula is deferred to the next time point).
At the beginning of the period, the current set~$\Fmc_{\fnow}$ is stored in $\Fmc_{s}$ and, until the end of the period, the algorithm continues the iteration as before. In addition, it however has to consider the $\Until$-subformulas deferred at time point~$s$ to make sure that they are satisfied within the period. If it has reached the end of the period, it checks if the latter is the case and if $\Fmc_{s}$, guessed for describing \altlint at the beginning of the period, can indeed fulfill that function.

Note that \cite{SiCl85:ltlpspace} do not regard the \Previous-operator, which is
considered by us. However, we can obviously assume that the sets of
subformulas that are guessed also include subformulas that include this operator and adapt the tests correspondingly (see the above specifications of $\algofont{\algoInitial}$ and $\algofont{\algoTCons}$). In particular, this does not affect the space requirements of the algorithm because the period that has to be guessed is still exponential in the
size of the considered formula.
%
Furthermore, we present the algorithm adapted to our setting, where satisfiability is to be decided w.r.t.\ time point~$0$. The original algorithm checks satisfiability at a time point given as argument.

We recapitulate the correctness and space complexity of the procedure. %, established in {\cite[Theorems 4.1 and 4.7]{SiCl85:ltlpspace}}.
%TODO 4.7. ref because we talk about the algo!
\begin{rwlemma}[{{\cite[\citethm4.1 and 4.7]{SiCl85:ltlpspace}}}]
	\label{prop:algo-ltl-sat}
	Algorithm~\ref{algo:ltl-sat} nondeterministically decides the satisfiability of a given LTL formula~\altlform by using an amount of space that is polynomially bounded in~$|\altlform|$.
\end{rwlemma}
